LLM-based Generation of Diverse and Realistic Domain Model Instances

Large Language Models (LLMs) have recently been proposed to support domain modeling tasks, mostly for the completion of partial models. However, another important task is the instantiation of domain models into concrete objects, which has received little attention. Existing generators focus on structural validity, but leave aside whether instances are realistic and diverse, although only such instances are understandable for humans and useful, e.g., for teaching modeling, for model-based testing, or as training data for machine learning. To address this gap, this paper presents LIMoGen (LLM-based Instance Model Generation), an approach that generates UML object diagrams from UML class diagrams with LLMs that use feedback from the USE model validation tool to repair malformed or non-conforming instances. We compare two prompting strategies, a single instruction-based prompt and a Chain-of-Thought strategy that steers the generation toward specific unusual scenarios, such as boundary, edge, and over-constraint cases. We applied LIMoGen to ten domain models and evaluated the generated instances for validity, coverage, diversity, and realism, the latter with domain-specific checks and an LLM-as-a-judge audited by human experts. The results show that all instances are well-formed, conforming, and diverse in values and structure. Most realism problems are inconsistencies between values, which the judge largely detects, as confirmed by the experts. Furthermore, we show that these findings help improve the domain models, as uninstantiated classes suggest abstract classes, over-constraint scenarios reveal multiplicities that are too strict, and realism problems uncover implicit domain knowledge that can be encoded as additional invariants.

==> preamble/packages.tex <==
\usepackage[utf8]{inputenc}
\usepackage{ifthen}
\usepackage{hyperref}

%\usepackage[dvipsnames]{xcolor}
\usepackage{mathtools}
\usepackage{soul}
\usepackage[normalem]{ulem}
\usepackage{graphicx}
\usepackage{pdfpages}
\usepackage{array}
\usepackage{epsf,picinpar}
\usepackage{varioref}
\usepackage{fdsymbol}
\usepackage{comment}
\usepackage{colortbl}
\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{fancyhdr}
\usepackage{multirow}
\usepackage{tabularray}
\usepackage{tablefootnote}
\usepackage{longtable}
\usepackage{tabularray}
\usepackage{tikz}
\usetikzlibrary{arrows.meta, positioning}
\usepackage{xfrac}
\usepackage{float} 
\usepackage{pgf-pie}

\usepackage{tikz}
\usepackage{subcaption}
\usepackage[title]{appendix}%
\usepackage{textcomp}%
\usepackage{manyfoot}%
\usepackage{booktabs}%
%\usepackage{algorithm}%
%\usepackage{algorithmicx}%
%\usepackage{algpseudocode}%
\usepackage{listings}%
\usepackage{tabularx}
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{pgfplots}
\mdfdefinestyle{rqanswer}{backgroundcolor=gray!10,roundcorner=3pt,outerlinewidth=1}

%\usepackage[most]{tcolorbox}
%\usepackage{algorithmic}
%\usepackage[ruled, linesnumbered, vlined]{algorithm2e}
%\usepackage[linesnumbered,lined,commentsnumbered]{algorithm2e}
%\usepackage{listings}

\usepackage{AMMALanguages}

\usepackage{makecell}
\usepackage{adjustbox}

==> preamble/settings.tex <==
%%%%%%%%%%%%%%%%%%% Show/hide annotations %%%%%%%%%%%%%%%%%%%
\newboolean{showannotations}
\setboolean{showannotations}{true} % TOGGLE TO SHOW ANNOTATIONS

%%%%%%%%%%%%%%%%%%% Show/hide names for double blind reviews %%%%%%%%%%%%%%%%%%%
\newboolean{shownames}
\setboolean{shownames}{true}

\pgfplotsset{width=10cm,compat=1.9}

%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%
%\newcommand{\newtextcolor}{Blue}
\definecolor{newtextcolor}{rgb}{0, 0, 1}
\definecolor{oldtextcolor}{rgb}{1, 0, 0}
\newcommand{\assignementcolor}{orange}
\definecolor{highlightcolor}{rgb}{.99, 1, .0}
\sethlcolor{highlightcolor}
\definecolor{darkred}{rgb}{0.6,0.0,0.0}

%%%%%%%%%%%%%%%%%%% Listings %%%%%%%%%%%%%%%%%%%
\lstset{
    basicstyle=\linespread{0.95}\footnotesize\ttfamily,
    columns=fullflexible,
    numberblanklines=false,
    numbers=left,
    numberstyle=\small\color{black},
    stepnumber=1,
    numbersep=5pt,
    backgroundcolor=\color{white},
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    frame=single,
    rulecolor=\color{black},
    tabsize=2,
    captionpos=b,
    breaklines=true,
    breakatwhitespace=false,
    xleftmargin=1.4em
}


==> sections/Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> sections/old/Validation-old-2.tex <==
\section{Evaluation}
\label{sec:validation}

In this section, we report on the evaluation of the presented instance generation approach, in particular, of the two prompting strategies introduced in Section~\ref{sec:approach}. We study whether they generate valid instances with respect to well-formedness and conformance, whether the resulting instance space is diverse, and whether the generated instances are plausible and consistent as snapshots of real-world domains. Since realism of values and structures cannot be captured by analyzing pure model information, we combine dedicated checks of values using additional information sources, an LLM-as-a-judge, an expert audit, and a subsequent model-refinement step.

\manuel{we should describe how we evaluate our approach: what is our method? Is it experiments in software engineering - cf. Wohlin?}

\subsection{Research Questions}


We aim to answer the following research questions:
\begin{questions}
    \item \textbf{How effective are the two prompting strategies in producing valid domain model instances?}
    \begin{questions}
        \item \textbf{Well-formedness:} To what extent do the generated instances comply with the plain object diagram syntax (i.e., comprising a valid graph structure)?
        \item \textbf{Conformance:} How accurately do the instances conform to the structural constraints, types, and multiplicities defined in the given domain model?
    \end{questions}

    \item \textbf{To what extent do the two prompting strategies generate diverse domain model instances?}
    \begin{questions}
        \item \textbf{Domain model coverage:} How effectively do the generated instances cover the elements defined in the underlying domain model?
        \item \textbf{Structural diversity:} How much structural variation exists among the generated instances?
        \item \textbf{Value diversity:} How effective are the strategies in generating a variety of concrete attribute values?
    \end{questions}

    \item \textbf{How effective are the two prompting strategies in producing realistic domain model instances?}
    \begin{questions}
        \item \textbf{Automated evaluation:} To what extent do automated domain checks and an LLM-as-a-judge classify the generated instances as realistic?
        \item \textbf{Human-based analysis:} What types of realism issues can be identified, and how reliably do the judge's assessments align with the assessments by humans?
        \item \textbf{Model refinement:} To what extent can the identified problems be formalized as additional OCL constraints that can be used to strengthen the underlying domain models?
    \end{questions}
\end{questions}

\subsection{Experimental Setup}
\label{sec:experimental-setup}

In the following, we describe the experimental setup of our evaluation, in particular the used domain models, the instance generation protocol, and the evaluation methodology, i.e., how we aim to answer each research question.

\subsubsection{Domain Models}

\input{tables/domains}

We have built a dataset of ten domain models from lectures taught by the authors and from ModelSet~\cite{LopezIC22-ModelSet}, taking into account $(i)$ different sizes, $(ii)$ variety of application domains, $(iii)$ the coverage of different modeling constructs such as constraints, $(iv)$  abstraction level (language level vs. concrete modeling level), and $(v)$ temporal or domain-specific reasoning, e.g, models which represent time or entail temporal constraints such as predecessor/successor relationships. 

Table~\ref{tab:characteristics} summarizes the main characteristics of the collected dataset. The number of model elements ranges from three classes in the Bank model to 22 in Restaurant model, from two attributes in the State Machine metamodel to 37 in Football model, and from three relationships in Bank and Videoclub models to 18 in Football model. Five models use inheritance relationships between classes and seven contain enumerations. The State Machine model is the only metamodel; the remaining nine models describe dedicated application domains. All models include OCL constraints, and six require some form of temporal reasoning.

Moreover, all models come with one or several domain-specific constraints
for the realistic values to be used in the instances. \manuel{we should describe it more. Some attributes are String/Integer typed but actually represent a more specific domain type. Some other parts are related to the afore mentioned temporal reasoning. For state machine we only say coherence....}

% The constraint counts in Table~\ref{tab:characteristics} refer to the original models supplied to the generator, before the model-refinement step described for RQ3.3.

\subsubsection{Generation Protocol}

\input{tables/llm-config}
\input{tables/instantiation}

% We used GPT-5.2 with the provider's default sampling parameters. 

% All instances were generated between 16 and 23 February 2026 with GPT-5.2 \texttt{(openai/gpt-5.2, snapshot: gpt-5.2-2025-12-11)} accessed through OpenRouter. We did not set sampling hyperparameters in the request, so OpenAI's GPT-5.2 defaults applied (\texttt{temperature}=1, \texttt{topP}=1, and \texttt{reasoning.effort}=\texttt{none}).
For each of the ten domains, we generated 30 instances with Instruction Learning (IL) and 30 with Chain-of-Thought (CoT), resulting in 600 instances. IL generates the 30 instances sequentially in one conversation. CoT performs six generation rounds, each producing one instance for each of five categories: baseline, complex, boundary, edge, and over-constraint detection. Thus, both strategies contribute the same number of instances per domain. The over-constraint category intentionally creates real-world scenarios that violate a multiplicity or an OCL constraint. Therefore this category is included when studying the complete output space, but excluded from dedicated analyses such as conformance validation as a violation is its intended outcome. Table~\ref{tab:llm-config} lists the LLM used, sampling parameters, and run dates.

Every tentative SOIL-based instance model was parsed and checked with USE and, except for violations explicitly requested in the over-constraint category, a failed check was returned to the generator for up to two feedback-based repair rounds. Table~\ref{tab:sizeGenInstances} reports the total numbers of objects, attribute assignments, and association links across the 30 instances generated for each domain and strategy.

% In total, IL generated 42,236 model elements and CoT generated 45,282, for 87,518 elements across both strategies.

% \manuel{we should talk here also about the LLM settings...}


% \manuel{we should check the paper from Wagner et al. about LLM usage and documentation in empirical studies.} 

% \manuel{https://llm-guidelines.org/checklist/}

\subsubsection{Evaluation Methodology}
\label{sec:eval-metrics}



% \paragraph{RQ1 - Validity}
% For \textbf{well-formedness} (RQ1.1), we count SOIL commands that USE cannot parse or execute. For \textbf{conformance} (RQ1.2), we count multiplicity and OCL-invariant violations reported by USE built-in checker after the repair loop. As explained above, the deliberately violating CoT over-constraint instances are not treated as failed attempts and are discussed in separation.

\paragraph{RQ1 - Validity}
First, we want to know whether a generated script is a valid instance of its domain model, or only resembles one. For that, we look at two complementary aspects. \emph{Well-formedness} asks whether USE can parse and execute the SOIL commands. \emph{Conformance} asks whether the object diagram that results satisfies the multiplicities and OCL invariants of the class diagram.
For \textbf{well-formedness} (RQ1.1), we count SOIL commands that USE cannot parse or execute.
For \textbf{conformance} (RQ1.2), we count multiplicity and OCL-invariant violations reported by USE built-in checker after the repair loop.

Let $E^{\mathrm{wf}}_i$, $E^{\mathrm{mult}}_i$, and $E^{\mathrm{inv}}_i$ be the well-formedness errors, multiplicity violations, and failed invariants USE reports for instance $i$. After the repair loop we report the sums (\ref{formula:rq1-errors}).
\begin{equation}
  E_{x}=\sum\nolimits_i |E^{x}_i|,\quad x\in\{\mathrm{wf},\mathrm{mult},\mathrm{inv}\}
  \label{formula:rq1-errors}
\end{equation}
CoT over-constraint instances are included in $E^{\mathrm{wf}}$ and excluded from $E^{\mathrm{mult}}$ and $E^{\mathrm{inv}}$.

\paragraph{RQ2 - Coverage and diversity}
For RQ2 we want to know whether repeated generation explores the instance space or repeats the same instance in disguise. For that, we look at three complementary aspects. \emph{Coverage} asks whether the instances use all elements of the model. \emph{Structural diversity} asks whether the object graphs differ and \emph{Value diversity} which asks whether the concrete values differ. In this case, attribute types call for different treatment. String, Integer, and Real attributes have large value spaces, so we measure pairwise distance between values. On the other hand, enumeration attributes have a small closed set of literals, where pairwise distance only tells whether two literals differ so we instead measure how evenly the literals are used. Lastly boolean attributes and custom data types (e.g., dates or time) are excluded from the pairwise metrics.

For \textbf{coverage} (RQ2.1), we compute, for every generated instance, the proportion of concrete classes, attributes, and associations of its domain model that it instantiates, and aggregate the values by domain and strategy.

Let $M_{\mathrm{cl}}$ be the set of instantiable classes of a domain model (abstract classes excluded), $M_{\mathrm{att}}$ the set of (class, attribute) pairs on those classes, with inherited attributes counted on each subclass, and $M_{\mathrm{rel}}$ the set of associations, compositions, and aggregations. For a generated instance $i$ and element type $t\in\{\mathrm{cl},\mathrm{att},\mathrm{rel}\}$, let $I_{i,t}\subseteq M_t$ be the elements that $i$ uses at least once: a $\texttt{!new}$ of that class, an assignment $\texttt{:=}$ of that attribute, or an $\texttt{!insert}$ into that relationship. 
The per-instance coverage is
\begin{equation}
  C_{i,t}=100\,\frac{|I_{i,t}|}{|M_t|}
  \label{formula:coverage}
\end{equation}

We report two aggregates per domain and strategy.
\emph{Within-instance coverage} is the mean and sample standard deviation of $C_{i,t}$ over the 30 instances.
\emph{Across-instance coverage} checks whether the 30 instances together reach every element, so
\begin{equation}
  C_t^{\mathrm{across}}=100\,\frac{\bigl|\bigcup_{i=1}^{30} I_{i,t}\bigr|}{|M_t|}
  \label{formula:coverage-across}
\end{equation}

% \manuel{Andrei, we may have to be careful here how the aggregation is done. Assume you have two instance which both have 40\% coverage, how is it aggregated? 40\% or 80\% or anything in between? I think we have to discuss again how this is actually computed and we should provide the concrete formulas here. BTW: maybe also for RQ1 we should provide formulas, even if they are simply sums of elements.}

% For \textbf{structural diversity} (RQ2.2), we represent every instance as an undirected labeled multigraph: objects are nodes labeled by their classes and links are edges labeled by their associations. We compute the pairwise Graph Edit Distance (GED) between the 30 instances generated for each domain and strategy, using unit-cost node and edge insertion, deletion, and label substitution. We normalize the raw distance as
% \begin{equation}
%   D_{\mathrm{GED}}(G_i,G_j)=
%   \frac{\mathrm{GED}(G_i,G_j)}
%   {\mathrm{GED}(G_i,\emptyset)+\mathrm{GED}(G_j,\emptyset)}
%   \label{formula:ged-diversity}
% \end{equation}
% Here, $\mathrm{GED}(G_i,G_j)$ is the minimum total cost of transforming $G_i$ into $G_j$ using the edit operations described above, and $\mathrm{GED}(G,\emptyset)=|V_G|+|E_G|$. We define $D_{\mathrm{GED}}(\emptyset,\emptyset)=0$. The resulting score is a normalized difference in $[0,1]$: 0 denotes structurally identical graphs, and larger values denote greater structural diversity. As GED is an NP-hard problem, exact GED values are used whenever the search completes within the configured time limit of 10 minutes. For a timed-out pair, we retain a certified interval $[L,U]$ and use its midpoint $(L+U)/2$ as an identified estimate.\manuel{we need citations for GED and the method we are using to show it is a meaningful way. It is also not clear what L and U are and how we get to these parameters...} Each cell in Table~\ref{tab:structural-diversity} summarizes the 435 unordered pairs of instances for a domain and strategy.\manuel{how is it summarized and why are we referencing now to the results? We should explain how we present the results in a general way.}

For \textbf{structural diversity} (RQ2.2), we represent every instance as an
undirected labeled multigraph: objects are nodes labeled by their class, and
links are edges labeled by their association keeping parallel edges between the same
two objects distinct. We use the unit-cost Graph Edit Distance
(GED)~\cite{SanfeliuFu83,RiesenBunke09}: each node or edge insertion, deletion,
or label substitution costs~$1$.
$\mathrm{GED}(G_i,G_j)$ is the minimum total cost of transforming $G_i$ into
$G_j$ under these operations, and
$\mathrm{GED}(G,\emptyset)=|V_G|+|E_G|$.
We normalize the raw distance as
\begin{equation}
  D_{\mathrm{GED}}(G_i,G_j)=
  \frac{\mathrm{GED}(G_i,G_j)}
  {\mathrm{GED}(G_i,\emptyset)+\mathrm{GED}(G_j,\emptyset)}
  \label{formula:ged-diversity}
\end{equation}
and set $D_{\mathrm{GED}}(\emptyset,\emptyset)=0$.
The score lies in $[0,1]$: $0$ denotes identical labeled graphs, and larger
values denote greater structural diversity.

Computing exact GED is NP-hard~\cite{BlumenthalBGBB20}, so for every pair we
compute a certified interval $[L,U]$ with $L\le\mathrm{GED}\le U$.
The upper bound $U$ is the cost of a concrete edit path, obtained by the
bipartite assignment (BP) of Riesen and Bunke~\cite{RiesenBunke09}, a single
IPFP descent~\cite{BougleuxBCFGV17} initialized from that assignment, and
swap-based local search (REFINE)~\cite{ZengTWFZ09,BoriaBBG20}.
The lower bound $L$ is BRANCH~\cite{BlumenthalGamper18}.
These heuristics are not symmetric in their two arguments, so we run both
orientations and keep the smaller $U$ and the larger $L$.
A pair is exact when $L=U$.
This combination is among the empirically tightest bound pairs in the survey
of Blumenthal et~al.~\cite{BlumenthalBGBB20}.
For each domain and strategy we summarize $D_{\mathrm{GED}}$ by the
mean~$\pm$~standard deviation over the $\binom{30}{2}=435$ unordered pairs
among the 30 instances, substituting $U$ for $\mathrm{GED}$ in
\eqref{formula:ged-diversity}.

For \textbf{value diversity} (RQ2.3), let $V=\{v_1,\ldots,v_n\}$ be the bag of attribute values of one type, numeric or string, under comparison. For within-instance diversity, $V$ collects the values of one instance and for across-instance diversity, it collects the values of all 30 instances of a domain and strategy.
% \manuel{are these the values stored in the model?}

We define diversity as the average distance over all unordered pairs:
\begin{equation}
  D_T(V)=
  \frac{1}{\binom{n}{2}}
  \sum_{1 \leq i < j \leq n} d_T(v_i,v_j),
  \qquad n \geq 2
  \label{formula:diversity}
\end{equation}
For numeric values and exact string comparison,
$d_T(v_i,v_j)=0$ if $v_i=v_j$, and $1$ otherwise.
For strings, we additionally use the normalized Levenshtein distance:
\[
d_{\mathrm{lev}}(v_i,v_j)=
\frac{\mathrm{lev}(v_i,v_j)}
     {\max(|v_i|,|v_j|)}
\]
Consequently, 0 denotes identical values and values closer to 1
indicate greater diversity.

We further assess the distribution of enumeration literals using normalized Shannon evenness~\cite{pielou1966}, which divides the Shannon entropy~\cite{shannon1948}
by its maximum possible value.
% \andrei{add a reference for this}
% \manuel{here it is now not clear why we do this only for enumeration. In particular for RQ2 we may describe a rational before we present the metrics - actually describe the measurement goal - what do we want to learn and then present the corresponding metric.} 
Let $\mathcal{L}=\{\ell_1,\ldots,\ell_m\}$ be the $m$
literals defined by an enumeration. For one enumeration-valued attribute in
one generated instance, let $c_j$ be the number of occurrences of literal
$\ell_j$, let $N=\sum_{j=1}^{m}c_j$, and let
$p_j=c_j/N$ when $N>0$. The set of active literals is
$\mathcal{A}=\{\ell_j\in\mathcal{L}\mid c_j>0\}$, with
$k=|\mathcal{A}|$. Its Shannon entropy is
\begin{equation}
  H=-\sum_{\ell_j\in\mathcal{A}}p_j\log_2 p_j
  \label{formula:shannon-entropy}
\end{equation}
If $N=0$, we define the entropy and both evenness scores as zero.
Entropy is zero when only one literal occurs and reaches its maximum when
the occurrences are uniformly distributed. We normalize the same entropy
using two different maxima:
\begin{equation}
  \begin{aligned}
    E_{\mathrm{active}} &=
    \begin{cases}
      H/\log_2 k, & k\geq 2\\
      0,          & k<2
    \end{cases}\\
    E_{\mathrm{all}} &=
    \begin{cases}
      H/\log_2 m, & m\geq 2\\
      0,          & m<2
    \end{cases}
  \end{aligned}
  \label{formula:shannon-evenness}
\end{equation}
Both scores lie in $[0,1]$. The active-literal score measures how evenly the
instance distributes occurrences among the literals it uses, whereas the
all-literal score additionally penalizes literals that it does not use. For
example, if an enumeration defines four literals but an instance uses two of
them equally often, then $H=1$, $E_{\mathrm{active}}=1$, and
$E_{\mathrm{all}}=1/2$. Thus, the selected literals are perfectly balanced,
but the instance covers only part of the enumeration.

We calculate both variants separately for every evaluated enumeration in
each of the 30 instances produced by each strategy. A domain has $r$
evaluated enumerations and $E_{ia}$ denotes either evenness score for
instance $i$ and enumeration $a$, Table~\ref{tab:enum-distribution} reports
the mean and sample standard deviation over the $q=30r$ scores:
\begin{equation}
  \begin{aligned}
    \overline{E}
      &=\frac{1}{q}\sum_{i=1}^{30}\sum_{a=1}^{r}E_{ia}\\
    s_E
      &=\sqrt{\frac{1}{q-1}
        \sum_{i=1}^{30}\sum_{a=1}^{r}(E_{ia}-\overline{E})^2}
  \end{aligned}
  \label{formula:shannon-aggregation}
\end{equation}

\paragraph{RQ3 - Realism}
For \textbf{automated evaluation} (RQ3.1), we use two complementary methods. First, we used domain-specific checks that validate selected values with regular expressions, libraries, external APIs, and cross-attribute comparisons. Examples include regular expressions for phone numbers, websites, email addresses, X (Twitter) usernames, and license plates; validators for IBANs and BICs\footnote{Bank-Account Validator, \url{https://gitlab.com/schegge-projects/bank-account-validator}}; API geocoding\footnote{Geoapify API, \url{https://www.geoapify.com/geocoding-api}} for addresses and coordinates; date comparisons; and the OMDb API\footnote{OMDb API, \url{https://www.omdbapi.com/}} for movies and series.

% Second, we submit each domain model together with each generated object model to Gemini 3.1 Pro through as an LLM-as-a-judge. The judge is instructed to assess common-sense plausibility and logical consistency, and to return one of \emph{realistic}, \emph{unrealistic}, or \emph{doubtful} label for the investigated object model, accompanied by a concise explanation of its reasoning. This provides a model-level assessment that complements the narrower executable checks. \manuel{we should provide here again details on the configuration of Gemini 3.1 Pro as well as where one can find the prompt which is used. And maybe we should explain in more detail what we ask for as an explanation for realistic and unrealistic models.}

The domain-specific realism checks serve as a general understanding of the realism of the values/attributes, but not of the realism of the instance as a whole, its structure, relationships, how they are connected and how the values relate to each other. For that we wanted something that evaluates the whole instances but also can be automated and scalable to further use in agentic pipelines. Our second method submits each domain model together with each generated instance to Gemini 3.1 Pro as an LLM-as-a-judge (see configuration in Table~\ref{tab:llm-config}). The system prompt frames the model as a software modeler performing ``semantic reality checking'': it must read the class diagram, map objects to classes, apply common-sense knowledge to values and relationships, and return one of \emph{realistic}, \emph{unrealistic}, or \emph{doubtful} together with a short justification that names the objects, values, or relationships that motivate the verdict. The prompt contains one worked example per label. The full prompt and all judge responses are available in~\cite{repo}.

For \textbf{human-based analysis} (RQ3.2), we drew a stratified random sample of 100 judge outputs. \manuel{we have to explain why we think the sample is enough... again, providing here a rationale what we want to analyse would be good before we go into the details.} The sample contained ten instances per domain, 50 per generation strategy, and 50 per judge verdict (realistic/unrealistic); within each verdict, 25 instances came from IL and 25 from CoT. Category was not an additional stratification factor as we prioritized balance across domain, generation strategy, and judge verdict: the 50 CoT cases comprised 15 baseline, 10 complex, 14 boundary, and 11 edge instances, with over-constraint instances intentionally excluded as they violate the model by construction and the judge is expected to call them unrealistic. Their conformance violations are reported in RQ1.2 and their judge verdicts in RQ3.1.
% \manuel{why are we exlcuding those and where do we analyse those?} 

The four authors reviewed the 100 judge outputs together in a synchronous meeting and assigned each statement a consensus veredict. For the 50 unrealistic verdicts, every reported problem was coded for two properties: whether the cited element exists in the instance (no LLM hallucination), and whether the problem is present (\emph{yes}, \emph{partial}, or \emph{no}). For the 50 realistic verdicts, explanations were split into specific statements (traceable elements in the instance) and generic statements (validity of the instance as a whole). These codes give problem-level and instance-level precision on the unrealistic half, a confirmation rate per domain, and traceability and validity rates on the realistic half.

Finally, for \textbf{model refinement} (RQ3.3), we use the confirmed problems from RQ3.2 to strengthen the domain models as many unrealistic instances are well-formed and conforming, so the missing knowledge sits in the class diagram, not in the generator. We group recurring problems and encode those expressible in OCL as additional invariants. We then re-check the 100 audited instances against the enriched models and compare the invariant verdict with the judge verdict and with the expert decision.

% \manuel{this is not setup but already the results. We have to move the result part to the next section and focus here on the evaluation methodology. For instace, we could state the ratio of issues which could be covered by OCL instead of having to resort to LLMs.}

\subsection{Results}
\label{sec:evaluation-results}

In this subsection, we present the results of executing the outlined experiment to answer the afore stated RQs. 

\subsubsection{RQ1 - Validity}

\input{tables/feedback}

\paragraph{RQ1.1 - Well-formedness}

\input{tables/taxonomy-wf}

Both prompting strategies produce well-formed object diagrams for every given domain model once the proposed repair loop has run. At command level, USE processed all 42,237 IL SOIL commands and all 45,282 CoT SOIL commands, and it needed only a small number of repair requests to do so.

Table~\ref{tab:llm-corrections} quantifies the repair effort behind these results. Across all domain models, USE well-formedness diagnostics triggered 9 correction calls for IL and 29 for CoT. Table~\ref{tab:wf-taxonomy} classifies the correction calls failures in four main categories: illegal syntax in USE, types mismatch, wrong links and boundary values.

CoT's deliberately invalid over-constraint instances received the same syntax repair as the other generated instances, and they are fully well-formed after it. Deliberately violating the model still seems to hurt the syntax, since 44\% (13 of the 29 CoT) of well-formedness repairs fall in this category.

\paragraph{RQ1.2 - Conformance}

\input{tables/taxonomy-cf}

The repair loop was also effective for conformance. The 300 IL instances produced no errors in 11,288 multiplicity checks and 900 invariant validations. After excluding the 60 over-constraint instances, the remaining 240 CoT instances also produced no errors in 10,370 multiplicity checks and 720 invariant validations.

Of the 60 over-constraint instances, 53 violate at least one multiplicity or invariant, 61 multiplicity violations and 26 invariant violations in total. The other 7 describe a scenario the LLM treated as over-constrained, although the model in fact permits it.

IL shows better well-formedness and CoT shows better conformance. This seems to come from how each strategy uses context. IL keeps one long conversation in which the shot and every accepted instance remain available, so the SOIL syntax stabilizes and few well-formedness repairs are needed. In that same conversation the LLM has to satisfy multiplicities and invariants without an explicit reasoning step, and that is where its 12 conformance repairs occur. CoT opens a fresh context per scenario and translates a natural-language description into SOIL, which costs more syntax repairs. The description step has already reasoned about multiplicities and constraints, so it makes sense that only three conformance repairs remain. Taking a closer look to the taxonomy of the conformance errors, we see that all 15 errors (12 IL + 3 CoT) are multiplicities failures, and as showed in Table~\ref{tab:conf-taxonomy} they can be classified in two main groups: Missing required link, ie. the object is connected to 0 things where the lower bound is at least 1 and Extra link, ie. the object is connected to 2 things where the upper bound is 1.


% \manuel{are all instances invalid?}

% \manuel{we have very low numbers here and not sure what it helps, but normally one would ask for pass@zereo, pass@one, etc. metrics.}


\begin{mdframed}[style=rqanswer,nobreak=true]
{\textbf{Answering RQ1:}} Both strategies produced fully well-formed SOIL outputs, and all instances conformed to their domain models. In the over-constraint category, 88\% of the 60 instances contain the intended conformance violations. More than 90\% of the instances were already well-formed and conforming on the first pass. USE feedback and the repair loop cover the rest.
\end{mdframed}

\subsubsection{RQ2 - Coverage and diversity}

\paragraph{RQ2.1 - Coverage}

\input{tables/coverage}

Table~\ref{tab:coverage} shows consistently high coverage, but no strategy dominates every domain. IL prompting shows class, attribute, and association coverage ranges from 87.1--100\%, 88.3--100\%, and 83.3--100\%, respectively. The corresponding CoT prompting coverage results ranges are 81.7--100\%, 80.6--100\%, and 85.3--100\% for classes, attributes, and associations, respectively. Both strategies cover every modeled class, attribute, and association in Bank. IL also reaches full coverage for all three element types in State Machine and Football, while CoT is particularly strong for Hotel Management. The lowest class and attribute coverage occurs for CoT on Videoclub; the lowest association coverage occurs for IL on Hotel Management and for CoT on Address Book. 
Hence, the union of the 30 instances per strategy reaches every element in nine domains. The gaps that remain can help us understand and improve the schemas. In Restaurant, the concrete superclass \texttt{Person} and its attribute \texttt{name} are never instantiated directly in any of the 600 instances, because the LLM always instantiates \texttt{Cook}, \texttt{Waiter}, \texttt{Manager}, and the other subclasses. A modeler would do the same, so \texttt{Person} is a candidate to be declared abstract rather than left concrete. \texttt{Cassette} in Videoclub is the same kind of signal. It is concrete, yet missing from 16 of the 30 IL instances and from 29 of the 30 CoT instances, which instantiate \texttt{Movie} and \texttt{Series} instead. Declaring it abstract would match how the domain is actually used. The other per-instance gaps are optional elements that depend on the scenario. \texttt{RoomExtra} is absent from 12 of the 30 IL Hotel Management instances, and \texttt{BusDriver} from 8 of the 30 IL Restaurant instances. Both appear in the union of those 30 instances, so they should probably stay in the model, but they are not classes that every scenario has to include.
% \manuel{what means repeated generation here.... more instances generated? instances improved? Also we should check if only optional elements (what is an optional element btw) are not covered. Why specialized elements are not covered? I thought the more general class is not covered when it is not set abstract? see the cassete example....}

\paragraph{RQ2.2 - Structural diversity}

\input{tables/ged}

Unlike coverage, structural diversity differs between the strategies (see Table~\ref{tab:structural-diversity}). Averaged over the ten domains, $D_{\mathrm{GED}}$ is 0.257 for IL and 0.410 for CoT, so CoT increases mean structural diversity by approximately 60\%. CoT is more structurally diverse in nine of the ten domains. The only exception is Hotel Management, where IL is slightly more diverse (0.353 versus 0.303). The largest difference occurs for Address Book (0.211 versus 0.561), followed by Vehicle Rental (0.256 versus 0.470) and State Machine (0.237 versus 0.445). Both strategies request diversity: the IL follow-up prompt asks for an instance that is structurally and semantically different from the previous ones, while CoT additionally prescribes a scenario category. The difference therefore measures the effect of explicit category steering (which seems to be more effective) on top of a generic diversity request. In particular, boundary, edge, and complex scenarios encourage changes in model size and topology that a generic diversity request does not specify.
\manuel{we also did not ask in IL for such scenarios? is it fair to compare?}
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/edge-bank.png}
  \caption{Edge instance generated with CoT for Bank (gen1). Every value is valid but
  unusual: banks in Monaco and Greenland (the latter without accounts), an owner aged 99
  next to one aged exactly 18, a 16-year-old account user, balances of 0 and 1, and
  names with diacritics. Both IBANs pass every automated check, yet a Monegasque bank
  holding a German and a French IBAN is incoherent (see RQ3.2).}
  \label{fig:edge-bank}
\end{figure}

Figure~\ref{fig:edge-bank} illustrates the effect of category steering. The edge instance is deliberately small (8 objects and 7 links, against an average of 13 objects and 20 links for the IL Bank instances) and includes a bank without accounts. Its mean $D_{\mathrm{GED}}$ to the 30 IL Bank instances is 0.40, compared with 0.25 among the IL instances themselves, so the metric places it clearly outside the region explored by IL.


\paragraph{RQ2.3 - Value diversity.}

\input{tables/diversity}

The value-level results in Table~\ref{tab:semantic-similarity} are high for all domains. Within instances, exact string diversity ranges from 0.9503 to 1.0000, while the normalized Levenshtein measure ranges from 0.7697 to 0.9068. Across instances, exact string diversity is at least 0.9978 and Levenshtein diversity ranges from 0.8155 to 0.9170. Numeric values show a similarly small amount of exact repetition: the within-instance scores range from 0.9173 to 0.9992 and the across-instance scores from 0.9158 to 0.9989, excluding Address Book, which has no numeric attributes. Per-strategy (IL vs CoT) aggregates differ by less than 0.01 for numeric and Levenshtein diversity, which motivates reporting their combined values. 

% \manuel{the previous sentence is not clear to me.}

\input{tables/shannon}

Exact-value diversity alone can hide concentration in small categorical domains. The Shannon results in Table~\ref{tab:enum-distribution} address this point. IL has higher evenness for both normalization schemes in five of the seven domains with evaluated enumerations, whereas CoT is higher in Videoclub and Restaurant. The largest difference in favor of IL occurs for Address Book (0.8981 versus 0.6980 for all literals), while the largest difference in favor of CoT occurs for Videoclub (0.5585 versus 0.7082). The two strategies therefore show no uniform advantage across finite alternatives: CoT's greater structural diversity does not imply a more even distribution of enumeration literals within individual instances.
\manuel{again in CoTs we were asking for different scenarios - maybe this also has an impact on eveness?}

% \manuel{BTW: we should explain in the setup that we have: String, Integer + Floats, Enums, and Booleans in models.... we consider all except Booleans - maybe they are too hard to consider... only two values... but at least we should discuss this in the experiment setup.}

\begin{mdframed}[style=rqanswer,nobreak=true]
{\textbf{Answering RQ2:}} Both strategies achieve similarly high model-element coverage and generate highly varied concrete values. CoT, however, provides substantially greater structural diversity due to explicit steering. Within-instance enumeration evenness remains broadly comparable, with domain-dependent differences and no uniform advantage across the two strategies.
\end{mdframed}

\manuel{overall this section is a lot about numbers - actually, how to interpret the different ranges of values, not clear to me. Are there any interpretation levels we can use?}

\subsubsection{RQ3 - Realism}

\paragraph{RQ3.1 - Automated evaluation}

\input{tables/errors-checks}
\input{tables/errors-judge}

% The domain-specific results in Table~\ref{tab:results} illustrate why realism requires more than a single metric and external validation means. Format-oriented checks are often successful. For instance, IL produces no invalid phone numbers, emails, realistic IBAN formats, countries, coordinates for accepted addresses, or X (Twitter) usernames. 

% However, checks for actual existence are much stricter. The IBAN reality check rejects 106 of 141 IL and 106 of 143 CoT values, and address lookup rejects 112 of 353 IL and 174 of 369 CoT addresses across the affected domains.\manuel{we can keep the real checks, but maybe we have to validate again that the IBAN checker is working as intended. Can we check all IBANS? Does it actually make a difference for our purposes?} Similarly, most generated Videoclub titles and actors cannot be verified through OMDb. These outcomes do not necessarily make a value implausible: fictitious but well-formed addresses, accounts, and productions are often preferable for privacy-preserving synthetic data. They substantiate the distinction between \emph{realistic} and \emph{real}.\manuel{this is a good point which should be discussed in more detail. We want realistic data, but not real data? What does it actually mean to have realistic data instead of real data...}

% Cross-attribute checks expose a different class of errors. IL produces no errors in the 1,508 dates covered by the generic date checks, while CoT produces 32 in 1,809. CoT additionally produces one inconsistent Hotel Management date comparison and one coordinate inconsistency. At model level, eight of the 30 IL State Machine instances and 15 of the 30 CoT instances are judged semantically incoherent by the dedicated check.\manuel{how is this done? In Table 8 we do not have entries for the state machine on the RHS?} These failures are not visible from isolated value formats.

% The LLM-as-a-judge overall classifies 215 of 300 IL instances as realistic (71.7\%) and 131 of 300 CoT instances as realistic (43.7\%); it does not use the doubtful label. The aggregate difference is explained in part by the CoT design. Baseline and complex CoT instances obtain realism rates of 46/60 (76.7\%) and 45/60 (75.0\%), respectively, which are close to the overall IL rate. By contrast, the boundary, edge, and over-constraint categories obtain 23/60 (38.3\%), 4/60 (6.7\%), and 13/60 (21.7\%), respectively. Thus, the judge results confirm that CoT successfully reaches unusual regions of the instance space, but these same regions more frequently violate common-sense expectations.\manuel{what are common-sense expectations?} The 13 over-constraint instances classified as realistic also show that the judge does not reliably replace formal conformance checking.\manuel{what does this mean - is the formal conformance checking showing for these instances problems the judge is overlooking? Should we also separate the CoT results for realistic checks - RHS of Table 8?}

% \andrei{Do we need to keep the real checks?}
% \andrei{want realistic data, but not real data? What does it actually mean to have realistic data instead of real data...}
% \andrei{Should we separate table 9, realism results in two: 1. realism rate Il + CoT by category and 2. realism checks Il + CoT by category (also)}

The LLM-as-a-judge realism rates for a whole instance are reported in Table~\ref{tab:realism-judge} and the number of values that pass a dedicated realism check in Table~\ref{tab:realism-checks}.

Real world rules and formats checks usually pass. IL has almost no invalid formatted phone numbers, emails, IBANs, BICs, countries and X usernames. However, stricter checks for the actual domain show that some generated values are not entirely valid. The IBAN(API) row checks the country prefix and the length, then the ISO 13616 check digits and the country-specific account structure. Only 35 of 141 IL and 37 of 143 CoT IBANs pass the full check. The failures are wrong check digits on otherwise well-formed IBANs, wrong lengths for the country, and IBANs invented for countries that don't use them, such as the US or Japan. Address lookup and OMDb show the same pattern. Addresses conform syntactically to addresses but do not resolve to real ones. For VideoClub IL finds 23 of 124 titles and 1 of 39 actors in OMDb. CoT finds 6 of 168 titles and none of 10 actors. 

These outcomes do not necessarily make a value implausible: fictitious but well-formed addresses, accounts, and productions are often preferable for privacy-preserving synthetic data. For teaching, testing, and training data, these values are still useful (see Figure \ref{fig:wf-iban-not-real}).

% \begin{figure*}[ht!]
%     \centering
%     \includegraphics[width=\linewidth]{figs/wf-address-not-real.png}
%     \caption{Well-formed but non-existent address in a Vehicle Rental instance generated with IL (gen23). The rental office \texttt{office\_callcenter10} has the address \texttt{`2000 Reservation Blvd, Wilmington, DE 19801'}, which follows the US address format and uses a real Wilmington ZIP code but the street does not exist, so address lookup fails.}
%     \label{fig:wf-address-not-real}
% \end{figure*}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\linewidth]{figs/wf-bank-not-real.png}
    \caption{Well-formed Bank instance generated with IL. All three accounts of the Spanish bank \texttt{Costa Sur Banco} have IBANs with the \texttt{ES} prefix and the correct length of 24, and the BIC \texttt{CSBKESMMXXX} is well formed. The bank, IBANs and its BIC are fictitious although they conform our checks.}
    \label{fig:wf-iban-not-real}
\end{figure*}

Comparisons between values in the same instance also pass. Every IL comparison in Table~\ref{tab:results} succeeds, including all 1,063 football dates and both Hotel Management date checks. CoT fails one Hotel Management checkout date comparison (31/32), three expense date ranges (59/62), 29 of 1,284 football dates, and one coordinate pair (64/65).

The judge labels 215 out of 300 IL instances as realistic (71.7\%) and 131 out of 300 CoT instances as realistic (43.7\%). It never uses the \textit{``doubtful''} label. Comparing by category, baseline and complex CoT perform similarly to IL, scoring 46/60 (76.7\%) and 45/60 (75.0\%), respectively. However, boundary, edge, and over-constraint categories are lower, at 23/60 (38.3\%), 4/60 (6.7\%), and 13/60 (21.7\%). These three categories are designed to be atypical, and the judge tends to score atypical instances as unrealistic. Thirteen over-constraint instances were labeled realistic; of these, 8 actually violated constraints, while the remaining 5 were described by the LLM as violations despite actually conforming to the model. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/ovc-example-hotel.png}
    \caption{Over-constraint instance Hotel gen5, labeled realistic by the judge. The room reservation has two bills (company and guest), which violates the multiplicity \texttt{1} of \texttt{BillRoomReservation}.}
    \label{fig:ovc-example-hotel}
\end{figure}

Analyzing these eight instances manually all of their violations are multiplicity violations. Hotel gen5 shows a typical case (see Figure \ref{fig:ovc-example-hotel}). Omar Al-Farsi stays one night on a business trip. His company pays for the rooms, and he pays for the parking and the minibar himself, so the single room reservation has two bills. Hotels split bills this way all the time. However, \texttt{BillRoomReservation} requires exactly one bill per room reservation. The same model already allows a booking to have several bills (\texttt{BookingBill} is \texttt{0..*}). It only forbids two of those bills from referring to the same reservation. The scenario is ordinary, and the judge is right to mark it as realistic and the domain model is overconstrained.

The other instances follow a similar pattern. Some violations show upper bounds that are too tight. In Football gen1 a team hosts two of its three cup matches, although \texttt{LocalMatch} allows only one. In Football gen3 a 17-year-old is registered with both the first team and the reserves. In Hotel gen1 a guest comes back for a second booking. Other violations show lower bounds that are too tight. Football gen5 has a match abandoned after 29 minutes because of lightning, which therefore has no report. Hotel gen1 has an empty room, and Restaurant gen4 has a table with no reservation. Expenses gen4 has a draft receipt and a comment not yet attached to an expense, although \texttt{DRAFT} is one of the model's own bill statuses. In Pickup Net gen5, a new shipment and a new customer have no station, and a rural delivery address described by landmarks has no geolocation. The \texttt{NEW} status and the optional driver suggest that a station could also be optional. Like the coverage gaps in RQ2, the over-constraint category therefore gives useful feedback to the modeller, helping to find constraints that are too strict, and it showing which parts of the model are easy to misread.

% \begin{table*}[ht]
% \caption{Over-constraint instances labelled realistic by the judge that violate the domain model. Multiplicities use USE notation and refer to the association end that is violated.}
% \label{tab:overconstraint-realistic}
% \centering
% \scriptsize
% \begin{tabularx}{\textwidth}{l|l|X|l}
% Instance & Violated association & Realistic scenario & Suggested \\ \hline
% Hotel gen5      & \texttt{BillRoomReservation} (\texttt{1})        & Company pays the rooms, guest pays the extras                    & \texttt{1..*} \\ \hline
% Hotel gen1      & \texttt{BookingCustomer} (\texttt{1})            & A guest books again three months later                           & \texttt{1..*} \\
%                 & \texttt{RoomReservationRoom} (\texttt{1})        & One room reserved twice, another not reserved                    & \texttt{*} \\ \hline
% Football gen1   & \texttt{LocalMatch} (\texttt{0..1})              & A team hosts two of its three cup matches                        & \texttt{*} \\ \hline
% Football gen3   & \texttt{TeamPlayer} (\texttt{1})                 & A youth player in both the first team and the reserves           & \texttt{1..*} \\ \hline
% Football gen5   & \texttt{MatchMatchReport} (\texttt{1})           & A match abandoned for lightning has no report                    & \texttt{0..1} \\ \hline
% Expenses gen4   & \texttt{ExpenseContainsBills} (\texttt{1})       & A draft rail ticket not yet assigned to an expense               & \texttt{0..1} \\
%                 & \texttt{ExpenseComment} (\texttt{1})             & A comment awaiting the supervisor's decision                     & \texttt{0..1} \\ \hline
% Pickup Net gen5$^\dagger$ & \texttt{StationShipment} (\texttt{1})  & A new shipment not yet routed to a station                       & \texttt{0..1} \\
%                 & \texttt{StationContainsCustomer} (\texttt{1})    & A new customer not yet assigned to a station                     & \texttt{0..1} \\
%                 & \texttt{AddressContainsGeoLocation} (\texttt{1}) & A rural address described by landmarks, without GPS              & \texttt{0..1} \\ \hline
% Restaurant gen4 & \texttt{ReservationTable} (\texttt{1})           & A table with no reservation                                      & \texttt{*} \\
%                 & \texttt{ChefCook} (\texttt{1}, \texttt{1..*})    & Chef and cook left unlinked (role names misread)                 & --- \\ \hline
% \end{tabularx}
% \\[2pt]{\footnotesize $^\dagger$Debatable: mandatory ownership links are a defensible design decision.}
% \end{table*}

% \andrei{I think (commented text down here) should be included somewhere. I dont know where (?) - because for human eval we did not take account over-constraints so there cant go, but also would be great to have instances examples also}
% Analyzing the 8 instances that were considered realistic but failed conformance, we can see some insights. For example, in GPT-5.2/CoT/Football/gen1/invalid, the FC København club features a single team: FCK First Team. This team plays three matches in the Nordic Invitational Cup 2026: at home against Malmö FF (January 14), away at IFK Göteborg (January 17), and at home against HJK Helsinki (January 20). Two of the three are home games. In our domain, the LocalMatch rule allows a team to play at home in at most one match, and VisitorMatch allows it to be away in at most one match. A second home match breaks LocalMatch, and a second away match breaks VisitorMatch. Since FCK First Team plays at home twice and away once, the LocalMatch multiplicity constraint fails, even though in real-life football scenarios, a team can have multiple home and away matches. This pattern also happens for the rest instances, in GPT-5.2/CoT/Hotelmag/gen1/invalid Aiko Tanaka stays from 10 March to 14 March, then again from 2 June to 5 June. Room 402 is used for both stays. Room 305 is empty. The domain model enforces that a guest can have only one booking, and that every room belongs to exactly one reservation. A guest who comes back, a room that is used again three months later, and a room that nobody has booked are all normal.

% Hotel, generation 5. Omar Al-Farsi stays one night. The company pays the room. He pays the minibar and the parking. That is two bills for one stay. The domain model says a reservation has exactly one bill. Hotels can split bills like this all the time. The same diagram already allows several bills on a booking, but forbids them to be for the same reservation inside that booking.

% Expenses, generation 4. Someone has a rail ticket from London to Cambridge, still marked draft. A comment says the supervisor has not decided whether it goes to Project A or Project B. The ticket and the comment are not attached to any expense. The diagram says every bill and every comment belongs to exactly one expense. The model's own statuses include draft. A receipt that has not been filed yet is a normal inbox.

% % Not sure about this one %
% PickupNet, generation 5. A parcel has just been created, status new, and no station has been chosen for it yet. The delivery address is a village in Bihar, described by a banyan tree and a handpump, with no GPS point. The customer who ordered it, Savitri Devi, is not assigned to a station either. The diagram says every shipment has a station, every address has a geolocation, and every customer belongs to a station. The status list already has 'new', a driver is allowed to be missing, and a rural address often has no reliable pin.
% % Not sure about this one %

% Restaurant, generation 4. Desert Pearl Café has an executive chef, Hiro Tanaka, and a cook, Ravi Kumar. They are not linked. The diagram says a chef supervises at least one cook, and a cook has exactly one chef. Both people are on the staff of the same café, so the realistic record is that Hiro supervises Ravi. The instance left that link out. That part is a hole in the instance, and the rule itself is a normal kitchen rule. The same instance also has table 31, an indoor booth, with no reservation, while two other tables are booked. The diagram says every table is in exactly one reservation. A café cannot draw its floor plan under that rule, because an empty table is not allowed, and this also mean a table cannot be booked twice. 

\paragraph{RQ3.2 - Human-based analysis}

\input{tables/judge}

For each instance the LLM as a Judge returns a verdict and a single explanation. Analyzing the 50 instances labeled unrealistic we split their explanations into 82 individual problems. Every object, value, or relationship named in a problem exists in the corresponding instance (i.e., they are traceable and there is no LLM hallucination inventing objects, relationships, or attributes the instance does not have). The experts fully confirm 60 problems and partially confirm seven, so 67 of the 82 problems (81.7\%) are accepted and 15 (18.3\%) are rejected and not considered actual instance issues. At instance level, 44/50 unrealistic verdicts contain at least one confirmed problem, whereas all reported problems are rejected for six instances. 

For the 50 instances labeled realistic, we split each explanation in the same way. This produced 198 statements, of which 63 are specific and 135 are generic. A specific statement names an object, value, or relationship (allowing us to evaluate traceability). A generic statement assesses the instance as a whole. All 63 specific statements refer to elements present in the object model (no LLM hallucinations inventing objects realtionships or attributes the instance does not have). Of the 135 generic statements, the experts accept 133. The two rejected statements occur in two different instances, so 48 of the 50 realistic verdicts contain no statement the experts reject.

In summary, we agree with the judge on 92 of the 100 audited instances. 

The taxonomy in Table~\ref{tab:expert-judge}\manuel{actually the table is not showing a taxonomy but categories which we have derived. I would also suggest to use a dedicated table for these categories.} shows that 39 of the 67 accepted problems (58.2\%) are logical inconsistencies, including temporal contradictions and cross-attribute violations. Plausibility issues account for a further 11 (16.4\%). The remaining findings concern missing domain constraints, modeling-language misinterpretations, domain-knowledge violations, and duplicated identities.\manuel{I will reframe this issues in three main categories: inconsistencies, plausibility issues, duplicates.} Agreement is domain-dependent (Table~\ref{tab:expert-judge-by-domain}): every reported problem is confirmed for Address Book, Expenses, and Restaurant, whereas only 37.5\% are confirmed for Bank. Typical false positives arise when the judge turns a convention into a universal rule, infers information not represented in the model, or assumes an unspecified unit or modeling paradigm. For example, a balance equal to the maximum 32-bit integer is unusual but not impossible, and a person's nationality cannot be inferred reliably from their name.\manuel{should we say that this also shows some biases?}

 
\paragraph{RQ3.3 - Model refinement}
The judge explanations and human adjudication provide actionable feedback about missing documented domain knowledge. We formalized recurrent, expressible domain rules as additional OCL invariants across all ten domain models. The invariants were written from problems in the audit, so they are aimed at unrealistic cases, but they were run on all 100 instances, to see if they detect the 2 instances marked as unrealistic by us, if they detect some additional unrealistic instances that we might have passed, or if they are to tight. \manuel{we should explain a bit more which invariants we have defined. Some are going beyond what is normally done with OCL.}

When applied to the 100 audited instances, the enriched models report at least one violation in 45 instances. The binary verdict of the new invariants agrees with the judge for 83/100 instances: 39 of the 50 instances labeled unrealistic fail at least for one added invariant, and 44 of the 50 labeled realistic models pass all of them. The remaining cases are informative in both directions.\manuel{I do not get this sentence...} Eleven judge-unrealistic instances pass the new constraints, reflecting semantic problems that the current formalization does not cover. \manuel{is this unexpected? we did not formalize all problems as OCL constraints}
Six judge-realistic instances fail an added invariant; these cases are candidates for either problems overlooked by the judge or constraints that are too restrictive and require expert review.\manuel{how does this align with the expert review and we should take a closer look at these instances why they fail - maybe the OCL constraints are too restrictive....}

\andrei{I think we should also analyze agreement human-ocl (see commented text)}
% The comparison that matters is OCL against the human labels. Agreement with the judge (83/100) mostly restates that the invariants were written from the same audit the judge had already flagged.

% From the 46(44+2) human labeled unrealistic 38 were ocl fails and 8 ocl passes
% From the 54(48+6) human labeled realistic 7 ocl fails and 47 ocl passes

%  Agreement ocl and the humans is 85/100. The interesting are:

% The eight that pass. Four of them are not really OCL constraints. Two are expressible and were just not written. Two sit in between.

% State names and time units are the ones OCL cannot see. statemachine gen6 baseline is an emergency landing that waits 180 seconds and then charges. Nothing in the model says what emergencyLanding or charging means. statemachine gen5 complex is the Unknown you counted as No: the judge said the durations are plausible in minutes, and the attribute has no unit. A bound would invent the unit.

% History and staffing are the ones you can write only by picking an arbitrary cutoff. myexpenses gen6 boundary is 28 February 1900, paid by credit card in South African rand. RealisticDates already allows any year from 1900 to 3000, so this date passes on purpose. Credit cards and the rand are facts outside the model. restaurant gen12 is one waiter for 120 guests. A ratio such as one waiter per 20 guests would fire, but the number would be ours, not the domain's. myexpenses gen25 is a refund stored as +6.00. category is a free string, and the object name is what says "refund". The sum invariant checks that the bills add up, and they do. The sign error is in the English, not in the structure.

% The two that were left out even though they are writable are bank gen1 edge and part of pickupnet gen5 boundary. The Monaco bank has DE and FR IBANs. ValidIbanCountry only checks that the prefix is some IBAN country, and both are, so it does not check that the prefix matches Bank.country. That match needs a table from country name to code. The pickup has an empty address string in the Pacific, which is a one-line invariant, and a North Pole to South Pole trip. The experts marked the trip Partial because the model never says whether a station is local, so that half should stay unencoded.

% hotelmanagement gen14 is the canceled, unconfirmed booking that still has late room service. "Canceled implies no on-site charge" is writable only if you keyword-match descriptions like "room service". "The dates are in the future" needs a clock the instance does not have.

% The seven that fail. Three are bad constraints. Two are real defects the experts did not review, because on a realistic verdict they checked the judge's sentences, not the rest of the instance. The last two are the same IBAN whitelist firing on a different issue than the one the experts rejected.

% addressbook gen1 complex fails SubdivisionBetweenCompanies for a mechanical reason. The invariant is a conjunction, not an implication, so every relationship that is not a subdivision fails it, including the bosses and employees in an instance the judge praised. CoworkerOnlyBetweenPersons is a separate, real hit: NordicAS is a coworker of AndesSpA, and several other companies are linked the same way. The explanation never mentioned that, so the audit did not either.

% hotelmanagement gen2 baseline fails Bill::SumOfExpenses. The formula charges every linked room for every night, then adds every extra: 3 nights times (180 + 140) plus 195 is 1155. The bill is 375. The model has no per-room dates, and the experts had just said that two rooms on one reservation is normal for a family. The invariant is stricter than the model can express. The 375 may also simply be wrong, and nobody checked the arithmetic.

% pickupnet gen18 fails AssignedShouldHaveDriver because shp_80005 is ASSIGNED and has no driver. The other assigned shipment does. The judge said the statuses line up, and the experts accepted that sentence. This one looks like a miss in the audit, not a tight constraint.

% The four bank failures are all ValidIbanCountry, and the whitelist is the problem. It omits AU, SG, US, KR, AR, CL, and MA.

% gen13 uses AU and SG. gen21 uses US. Those countries do not issue IBANs. The judge and the experts treated a matching prefix as enough, so the constraint is stricter than the audit.
% gen16 uses KR and AR, which also are not IBAN countries. The experts were rejecting a different claim, that nationality can be read off a name. They never scored the IBANs.
% gen20 uses MA and CL. Morocco and Chile do issue IBANs. They are missing from the list, so this failure is a hole in the registry, not a bad instance.

The refinement therefore converts a large portion of qualitative feedback into executable domain knowledge and exposes underspecification in the original class diagrams. Nevertheless, this step is an exploratory assessment on the same sample from which the constraints were derived. We did not regenerate instances using the enriched models. The results therefore demonstrate that the models can be strengthened and that future generations could receive more precise feedback, but they do not measure whether regeneration with the additional constraints improves realism.\manuel{maybe we move this part to the threats to validity as we answer the RQ, but of course, we could do more in the future...}

\begin{mdframed}[style=rqanswer,nobreak=true]
{\textbf{Answering RQ3:}} Realism depends strongly on both the domain and the requested scenario. IL and the baseline/complex CoT categories usually produce plausible instances, while boundary and edge steering deliberately exposes many unrealistic but conforming cases. Gemini 3.1 Pro provides grounded and useful findings, with 81.7\% of its reported problems fully or partially confirmed, but it also makes domain-dependent assumptions. The 48 newly declared OCL invariants flag 45 of the 100 audited instances and agree with the judge on 83\%, showing that judge feedback can guide domain-model refinement but cannot replace either formal validation or expert judgment.
\end{mdframed}

\subsection{Threats to Validity}

We discuss conclusion, construct, internal, and external validity following Wohlin et al.~\cite{WohlinRHCB12}.

\subsubsection{Conclusion Validity}

LLM generation and LLM-based judging are non-deterministic. We mitigate this threat by generating 30 instances for every domain and strategy and by reporting distributions or standard deviations where applicable. Still, the study is descriptive and does not claim statistical superiority for every metric. The expert sample is balanced by design; consequently, its agreement rates characterize the selected strata but must not be interpreted as prevalence or overall accuracy under the original distribution of realistic and unrealistic verdicts. In addition, the sample size becomes small when divided by domain, strategy, verdict, and CoT category, and the sampled CoT cases do not cover the over-constraint category.

\subsubsection{Construct Validity}

Each measure operationalizes only part of the intended construct. High coverage does not imply diversity, and high GED diversity does not imply meaningful variation. Our GED abstraction ignores attribute values and represents associations as undirected edges. Conversely, the value-difference metrics quantify repetition but not whether the values represent appropriate demographic or statistical distributions. The domain-specific realism checks cover only selected attributes and mix checks of plausibility with checks of actual existence. Finally, an LLM-as-a-judge is a proxy for the inherently contextual notion of realism. We therefore triangulate these measures instead of treating any one of them as ground truth.

\subsubsection{Internal Validity}

The prompts, examples, repair policy, and choice of GPT-5.2 may influence the results. USE feedback is part of the treatment and explains why final syntactic and conformance performance is stronger than raw generation performance. The four human reviewers saw the judge explanations and reached decisions jointly. Consensus enabled discussion of domain-specific ambiguities, but it may anchor the assessment and does not provide independent ratings from which inter-rater agreement can be calculated. Most importantly, the additional OCL constraints were derived from and reevaluated on the same 100-instance sample, and no instances were regenerated with the enriched models. The 83\% agreement therefore measures formalization of observed issues, not out-of-sample predictive performance or improved generation. A future study should use an independent holdout set and, if individual ratings are collected, report inter-rater agreement.

\subsubsection{External Validity}

The dataset contains ten heterogeneous models, but they are relatively small and largely drawn from educational contexts. Results may differ for industrial-scale models, specialized domains with limited public knowledge, or other modeling languages. We also evaluate one generator model (GPT-5.2) and one judge model and version (Gemini 3.1 Pro preview). Both model behavior and hosted implementations may change, and the conclusions cannot be transferred directly to other LLMs. Finally, the CoT strategy deliberately includes boundary, edge, and over-constraint scenarios; its aggregate realism rate should therefore not be generalized to workflows that request only typical instances.


==> sections/old/Validation-old.tex <==
\section{Evaluation}
\label{sec:validation}

% To have in the radar: On the Effectiveness of LLM-as-a-judge for Code Generation and Summarization https://arxiv.org/pdf/2507.16587

In the following, we report on the results of a systematic evaluation of our approach with respect to the two prompting strategies. Specifically, we evaluate to what extent our approach is capable of automatically generating semantically diverse and realistic domain model instances.

\subsection{Research Questions}
We aim to answer the following research questions:
\begin{questions} 
    \item How effective are the two prompting strategies in producing syntactically correct model instances w.r.t. the following two aspects: RQ1.1: well-formedness of the plain object diagram syntax; RQ1.2: conformance with the given domain model?
    \item How effective are the two prompting strategies in producing diverse domain model instances, from a structural point of view and from the values point of view? RQ2.1 How effectively do the two prompting strategies ensure coverage of the domain model when generating instances? \lola{New RQ}. RQ2.2 tbd other interesting structural aspects (graph similarity etc)

    \item How effective are the two prompting strategies in producing realistic \todo{rationally sound having the domain constraints, domain knowledge, domain experience reflected} domain model instances?

    %% maybe we can also cite https://dl.acm.org/doi/epdf/10.1145/3654777.3676450
    
    %% RQ3.1
    %% 1. llm as a judge evaluation with comments - base metric realistic / unrealistic models
    %% 1.1. At first we wanted to evaluate the instances realism ourself - but we did not agree
    %% 1.2 So then we decided to analyze the judge comments:

    %% RQ3.2
    %% 2. analyze the judge comments - validation on a sample - agreement scales @Lola 
    %% computed sample metrics, open process - knowledge generating process -
    %% categorization about the problems
    %% hallucinations

    %% RQ3.3
    %% subquestion of RQ3 - what can you do now to improve our models
    %% 3. obtain additional ocl constraints 
    %% 4. reevaluate
    %% problems found, agreement, ...
    
    % \item To what extent are the two prompting strategies able to scale with an increasing size of models and model instances?\todo{both are still open, but IMHO it would be amazing to test both at least with a few experiments}
\end{questions}

\subsection{Experimental setup \lola{to update by: Andrei}}

\subsubsection{Tool configuration}
For all our experiments, we set the number of instances to be generated to 30 (numInstances = 30) and the maximum syntax checks based on USE to two rounds (maxChecks = 2).

\subsubsection{Domains}
We have built a dataset of domain models by selecting models from lectures held by the authors of this paper, and from ModelSet~\cite{LopezIC22-ModelSet}, taking into account: 1) size, 2) a variety of domains, 3) the presence of constraints, 4) abstraction level (meta-level such as the state machine metamodel vs. non-meta-models such as the address book model), 5) requiring temporal reasoning (i.e., models which can represent time or entail temporal constraints such as
predecessor/successor relationships such as the hotel management model).

Table~\ref{tab:characteristics} presents the main characteristics of each selected domain model. %Note that even if these examples contain other model elements (such as datatypes and abstract classes)\lola{todo}, for space reasons, we have not added this information to the table. 
The number of classes and relationships across all domain models ranges from three classes of the Bank model up to 22 classes for the Restaurant domain, and three relationships for the Bank and Videoclub models up to 18 for the Football model. The number of attributes ranges from two attributes for the State Machine meta-model up to 37 attributes for the Football model. Five out of the ten domain models have at least two inheritance relationships, moreover, seven domain models entail at least one enumeration. One model is on the metamodel level, while the others are on the model level. All our models have at least one constraint, the Vehicle Rental model with five constraints has the most. Our dataset has six models that entail temporal reasoning. Moreover, all models come with one or several domain-specific semantic constraints for the values to be used in the instances.

\begin{table*}[]
\vspace{-.3cm}
\caption{Characteristics of the domain models used for the evaluation}
\label{tab:characteristics}
\begin{minipage}{\textwidth}
  \centering
\begin{tabularx}{\textwidth}{l|p{.4cm}p{.6cm}p{.5cm}p{.5cm}p{.5cm}lp{.4cm}|l|p{.45cm}|p{.45cm}|l}
\multicolumn{1}{c|}{\multirow{2}{*}{Domain}} & \multicolumn{7}{c|}{Size (Number of elements)}                                                       & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Abstr.\\ Level\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{Constr.}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Temp.\\ Reas.\end{tabular}}} & \multirow{2}{*}{Domain Semantics\footnote{Note that we only list those attributes here for which we defined semantic checks}} \\
\multicolumn{1}{c|}{} & Class & Abst.Cl & Attr. & Rel. & Inh. & Enum & Dt & & & & \\ 
\hline
Address Book    & 7  & 0 & 14    & 5    & 2    & 2 & 1  & model     & 1       & No & Phone, website, email, address        \\ \hline
Bank & 3  & 0 & 8     & 3    & 0    & 0 & 0  & model     & 2       & No & IBAN, BIC code, country    \\ \hline
Hotel Management& 7  & 0 & 22    & 6    & 0    & 0 & 0  & model     & 3       & Yes& Dates (checkin\textgreater{}=start, checkout\textless{}=end)       \\ \hline
Expenses        & 5  & 0 & 11    & 3    & 0    & 2 & 1  & model     & 2       & Yes& Dates    \\ \hline
Pickup Net      & 6  & 0 & 10    & 8    & 0    & 1 & 0  & model     & 4       & No & Address, latitude, longitude, X username       \\ \hline
State Machine   & 5  & 1 & 2     & 6    & 3    & 0 & 0  & metamodel & 2       & Yes& Coherence\\ \hline
Vehicle Rental  & 8  & 1 & 27    & 5    & 3    & 1 & 1  & model     & 5       & Yes& Address, license plate, valid home phone       \\ \hline
Videoclub       & 7  & 1 & 11    & 3    & 2    & 1 & 1  & model     & 3       & Yes& \begin{tabular}[c]{@{}l@{}}Production title, genre, type (movie or\\ series), actors, rental year \textgreater release year\end{tabular}       \\ \hline
Football        & 16 & 0 & 37    & 18   & 0    & 8 & 0  & model & 4  & Yes & \begin{tabular}[c]{@{}l@{}}Player name, Club name, Team name,\\ Competition name, Start date, End date\end{tabular} \\ \hline
Restaurant      & 22 & 2 & 34    & 13   & 11 & 8 & 2  & model & 4 & No  & \begin{tabular}[c]{@{}l@{}}Person name, Restaurant name, \\Phone number, Driverlicense number, \\Menu item, Food item, Date\end{tabular} \\ \hline
\end{tabularx}
Abstr.Cl = Abstract Classes, Attr. = Attributes; Rel. = Relations; Inh. = Inheritance; Enum = Enumerations; Dt = Datatypes; Abstr. Level = Abtraction Level; Temp. Reas. = Temporal Reasoning
\end{minipage}
\vspace{-.3cm}
\end{table*}


\subsubsection{Evaluation metrics}\label{sec:eval-metrics}
\input{tables/sizeGenInstances}


We used to the following evaluation metrics to respond to the previously introduced research questions: 
\begin{description}
    \item[Well-formedness (RQ1.1):] We evaluate how many of the generated model instances expressed in the textual object diagram syntax can be parsed by USE.
    \item[Conformance (RQ1.2):] We evaluate how many conformance errors are reported when validating the generated model instances with USE i.e., how many typing, multiplicity, and constraint violations are reported.
    \lola{I've checked up to here. To  be continued...}
    \item[Semantic correctness (RQ2):] Whenever possible, we implemented automated semantics checks based on existing APIs or regular expressions (RegEx). In exceptional cases, we conducted a manual semantics check. 
    All our semantic checks can be differentiated based on whether they check variables for being \texttt{realistic} or \texttt{real}.
    The following checks for \texttt{realistic} attribute values were used: Phone number: we developed a RegEx; Website: we developed a RegEx, Email: we developed a RegEx, Address: we used an existing API\footnote{\url{https://www.geoapify.com/}}; IBAN, BIC: We used an existing validator\footnote{\url{https://gitlab.com/schegge-projects/bank-account-validator}};  X Username: we developed a RegEx; License plate: we developed a RegEx; 
State machine: we manually checked the semantic coherence of terminology used the state machine described by the instance model; Videoclub properties: production title, genre, type, actors, and release date were validated an existing API\footnote{\url{https://www.omdbapi.com/}}.
    %\begin{description}
     %   \item[Phone number:] We developed a RegEx.
      %  \item[Website:] We developed a RegEx.
      %  \item[Email:] We developed a RegEx.
      %  \item[Address:] We used an existing API\footnote{\url{https://www.geoapify.com/}}.
      %  \item[IBAN, BIC:] We used an existing validator\footnote{\url{https://gitlab.com/schegge-projects/bank-account-validator}}.
       % \item[X Username:] We developed a RegEx.
       % \item[License plate:] We developed a RegEx.
       % \item[State machine:] We manually checked the semantic coherence of terminology used the state machine described by the instance model. 
       % \item[Videoclub properties:] Production title, genre, type, actors, and release date were validated an existing API\footnote{\url{https://www.omdbapi.com/}}.  
    %\end{description}
    %Further, the following checks for \texttt{real} attribute values were used:
    %\begin{description}
     %   \item[Address:] We manually assessed whether addresses exist.
      %  \item[IBAN, BIC:] We used a RegEx and tested the validity of the checksum.
       % \item[Country:] We used an existing API\footnote{\url{https://docs.oracle.com/javase/8/docs/api/java/util/Locale.html}}
        %\item[Dates:] We used the Java \texttt{java.time.LocalDate} implementation and an existing comparator\footnote{\url{https://docs.oracle.com/javase/8/docs/api/java/time/LocalDate.html}} 
        %\item[Latitude and Longitude:] We used an existing API\footnote{\url{https://www.geoapify.com/}}.
    %\end{description}



Further, the following checks for \texttt{real} attribute values were used: Address: we manually assessed whether addresses exist; IBAN, BIC: we used a RegEx and tested the validity of the checksum; Country: we used an existing API\footnote{\url{https://docs.oracle.com/javase/8/docs/api/java/util/Locale.html}}; Dates: we used the Java \texttt{java.time.LocalDate} implementation and an existing comparator\footnote{\url{https://docs.oracle.com/javase/8/docs/api/java/time/LocalDate.html}}; Latitude and Longitude: we used an existing API\footnote{\url{https://www.geoapify.com/}}.

    
    %This has been achieved, amongst others, by calling external and open-source APIs to check whether a movie title exists and who its actors are (for the Videoclub model) or writing a function that checks the well-formedness of an IBAN (for the bank model) or an X username (for the Pickup Net model). All semantic checks we realized can be found online\textsuperscript{\ref{foot:supp}}; the results of their evaluation are summarized in Table~\ref{tab:results}.
    %\todo{here we should add a list of all we did to check sem correctness, maybe a listing or even a table} \todo{very interesting metric, again, we should count the violations of realistic model elements/values, etc. A few further points: is the IBAN actually semantic or syntactic? we could also talk about reliability. Maybe in the threats to validity we should also say that we did not evaluate recall and accuracy or other metrics which may be used for other purposes... or is accuracy?}
    \item[Semantic diversity (RQ3):] We calculate a semantic diversity score within instances and across instances.  Within instances, we form a bag with all attribute values of the same kind (i.e., numeric or string) and compute the diversity score of these bags. Across instances, we put all the attribute values of all the instances of a domain into a bag, and compute their diversity score. The formulas for the numeric types are given below. %Note, that we use the same formula for computing the diversity of string types except that we use the normalized Levenshtein distance and an exact match in the sum function of the numerator:

%Numeric diversity:
% In math notation:
{\small
\begin{equation}
\label{formula:diversity}
    \forall x_i,x_j \in elems \text{ diversity}_\text{type} = \frac{\sum d(x_i,x_j)}{\frac{|elems|^2-|elems|}{2}}
\end{equation}
    
}
where $i\neq j$, $x_i \leq x_j$ , \emph{type} $\in \{String, Numeric\}$, \textit{elems} is the set of all attributes of kind \emph{type} in the model and \emph{diversity($x_i$,$x_j$)} is given by the following formulae:

{\small
\begin{equation}
d(x_i,x_j)= \left\{ \begin{array}{lcc} 1 & if & x_i = x_j \\ 0 & if & x_i \neq x_j \end{array} \right.
\end{equation}
}
% \lola{we can unify the two formulas for numbers and string, they are the same except what's inside the sum that is:
% s(xi,xi) for numbers; and nlev(xi,xj) or xi=xj for strings}

% % String similarity
% {\small
% % In math notation:
%     $$\forall x_i,x_j \in elems \text{ sem\_similarity}_\text{string} = \frac{\sum nlev(x_i,x_j)}{\frac{|elems|^2-|elems|}{2}}$$ 
% }
Note that for the \emph{String} type the operator $<$ represents the lexicographical order of the characters that form the strings. 
Further, the Levenshtein distance (\emph{lev}) is a very well-known and widely used metric to measure word similarity. It calculates the distance between two words as the minimum number of single-character edits (insertions, deletions, or substitutions) required to change one word into the other. In addition to the formula \ref{formula:diversity}, which calculates diversity using the exact word match, in this work, we have defined an additional diversity metric that uses the Levenshtein distance. To be able to make comparisons, we used the normalized Levenshtein distance and, since \emph{lev} measures similarity and not diversity, we calculate the complement (a.k.a. inverse) of the normalized value. The formula is as follows:
{\small
\begin{equation}
d(x_i,x_j)= 1 - \frac{lev(x_i,x_j)}{max(length(x_i), length(x_j))}
\end{equation}
}

% Basically, we put all the attributes in a bag, we calculate the similarity of each pair, add all these values and we divide the sum by the number of pairs.
% elems = {...}
% sum = 0
% for (int i=0; i<elems.size(); i++)
%   for (int j=i+1; j<elems.size(); j++)
%       sum += nlev(elems[i], elems[j]) // o exact match with equals()
% return sum / elems.size()
    
    % \item[Scalability] \todo{depends on the RQs - currently we do not have a RQ for scalability.} We evaluate whether our approach scales with the generation of model instances of different sizes, i.e., small (0-15 elements), medium (15-50 elements), and large (50-100 elements). Particularly, we evaluate the relationship between the number of semantic errors with respect to the size of the model (i.e., $\frac{\# \text{ semantic errors}}{\text{model size}}$). 
    %\item Number of tokens (this could be useful to compare between different strategies). There is a trade-off. The greater the number of tokens the more expensive (computationally and financially) and sustainable the approach. Also, approaches that use more tokens (e.g., such as CoT wrt single instruction learning) get better results. \lola{right now we're not reporting the number of tokens but we could easily do it.} 
    % \item elapsed time (i.e., the time the generation took) \lola{we said we were not going to add this.}
\end{description}

\subsection{Results}

\andrei{Explain our thought process about not evaluating the judge, we first evaluated the instances ourself we did not get to conclusions, realism is subjective, so then we decided to categorize and analyze the judge issues. Give the example about the Bank - IBAN ES of a German bank - Manuel}

Table~\ref{tab:sizeGenInstances} provides an overview of model instances we generated following the two strategies we introduced in Section~\ref{sec:approach}. Note, that these are the number of elements generated in total for all 30 instances per domain. It can be derived that generally, the Chain-of-Thought (CoT) strategy generates instances of significantly larger size compared to the Instruction Learning (IL) strategy for most of the cases. 
In the following, we respond to each of the research questions individually. 

\subsubsection{RQ1 - Syntactical correctness}
Table~\ref{tab:results} (see columns 2-5) summarizes the results of the syntactic evaluation of the generated domain model instances. 
It can be seen that zero syntactic errors were found across all 300 model instances that were generated by applying the IL strategy. For the CoT strategy, we identified, in total, only three syntactic errors for 1698 generated model elements in instances of the Vehicle Rental domain and nine syntactic errors for 3618 generated model elements in instances of the Restaurant domain. 
Note that the table reports the errors found in all generated model elements (e.g., object creation, attribute initialization, association creation) of the 300 model instances generated with the IL strategy and 240 model instances generated with the CoT strategy. The instances generated in the over-constraint detection category are intentionally omitted as we forced the LLM to violate constraints.
% \manuel{a few questions: 1) we have 10 domain models, 30 instances generated per domain model, should sum up to 300 models?} \lola{I think we have already clarified this. We are not counting the models for overconstraint detection.}
% \manuel{What about the syntactic errors in the restaurant model? BTW: for the syntax errors we said in the metrics we count the number of models which have syntax problems, now we have 3/1698 and 9/3618 - what are the numbers?} \lola{this is the number of model elements (object creation, attribute initialization, association creation) that produced syntax errors}

When looking at the conformance of instances with respect to the domain models, we can also see that the IL strategy acted without producing errors in all 300 generated instances. The CoT strategy produced very few model element errors in the generated instances of Hotel Management (six out of 261), Expenses (three out of 48), Football (two out of 143), and Restaurant (14 out of 617) domain models.


\begin{mdframed}[style=rqanswer,nobreak=true]
{\textbf{Answering RQ1:}} Both prompting strategies can effectively generate syntactically correct instances considering the well-formedness of the object diagrams and their conformance to the domain models.
\end{mdframed}

\input{tables/table-results}

\subsubsection{RQ2 - Semantic correctness}
When looking at the domain semantics analysis summarized in Table~\ref{tab:results} (see columns 6 and 7), we can see that the results for the semantic correctness of the generated instances are more nuanced.
The table reports the number of model elements that have passed our semantic checks with respect to the total number of elements generated of that kind. 
Note that we separate checks on \texttt{realistic} property values (presented in standard font in Table~\ref{tab:results}) from those for \texttt{real} property values (presented in \textit{italics} font in Table~\ref{tab:results}).

We see that the LLM is capable of generating well-formed addresses and structural properties like phone numbers, email addresses, and license plates without a single error. When checking whether an address exists in reality, we encountered 152 errors in 194 model elements in the LLM-based generation in both strategies. Similarly, the generation of well-formed IBANs was mostly successful (only 10 errors in 169 model elements), while a reality check resulted in 83 errors in 90 model elements using IL and 73 errors in 79 model elements using CoT. 
A possible explanation could be related to privacy, i.e.,\ that the LLM is configured to intentionally omit real values for sensitive properties.
% \todo{do we have an idea why this is the case? maybe they intentionally shall not create real addresses/IBANs?} \lola{discuss privacy at some point in the paper. Provide examples everywhere, which was a violated IBAN, violated, ...}. 
Temporal reasoning was excellent in both strategies. When summarizing all time-related constraints like \textit{checkIn \textless{} checkOut} or \textit{Rental year \textgreater{} Release year}, we only encountered two errors across all 849 time-related property value generations. 

Until now, we primarily focused on realistic semantics on individual property value levels. However, the two prompting strategies were also very effective in creating semantically coherent models. When checking the combination of the property values generated for all generated State Machine model instances, we only found a single model (out of 54) that was not semantically coherent.

% \todo{should we provide some erroneous examples here or only discuss this with the sample models}

\begin{mdframed}[style=rqanswer,nobreak=true]
{\textbf{Answering RQ2:}} Overall, both prompting strategies showed effectiveness in creating realistic property values across domains. A significant decrease in the generation quality was assessed when checking whether the values were real. Both strategies were also effective in generating semantically coherent models.
\end{mdframed}


%\begin{table*}[]
%\centering
%\scriptsize
%\caption{Graph similarity}
%\]label{tab:graphSimilarity}
%\begin{tabular}{l|l|llllll}
%\multicolumn{1}{c|}{\multirow{2}{*}{Domain}}               & \multicolumn{1}{c|}{Instr. Learn.} & \multicolumn{6}{c}{Chain of Thought Learn.}                                                    \\ \cline{2-8} 
%\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{All}              & \multicolumn{1}{c|}{All} & \multicolumn{1}{l|}{Base} & \multicolumn{1}{l|}{Complex} & \multicolumn{1}{l|}{Boundary} & \multicolumn{1}{l|}{Edge} & Over-constraint \\ \hline\hline
%Address Book                                               &  0.99$\pm$0.02                 & \multicolumn{1}{l|}{0.92$\pm$0.04}    & \multicolumn{1}{l|}{1$\pm$0}     & \multicolumn{1}{l|}{0.97$\pm$0.02}        & \multicolumn{1}{l|}{0.92$\pm$0.05}         & \multicolumn{1}{l|}{0.99$\pm$0.01}     & 0.93$\pm$0.5                \\ \hline
%Bank                                                       &   $0.97\pm0.06$                          & \multicolumn{1}{l|}{$0.86\pm0.11$}    & \multicolumn{1}{l|}{$0.88\pm0.08$}   & \multicolumn{1}{l|}{$0.95\pm0.04$}  & \multicolumn{1}{l|}{0.94$\pm0.03$}        & \multicolumn{1}{l|}{$0.95\pm0.03$}       &  $0.93\pm0.06$               \\ \hline
%Hotel Management &     $0.95\pm0.04$                        & \multicolumn{1}{l|}{$0.74\pm0.16$}    & \multicolumn{1}{l|}{$0.83\pm0.12$}     & \multicolumn{1}{l|}{$0.83\pm0.14$}        & \multicolumn{1}{l|}{$0.76\pm0.17$}         & \multicolumn{1}{l|}{$0.96\pm0.03$}     &  $0.72\pm0.13$               \\ \hline
%Expenses                                                   &   $0.94\pm0.11$                          & \multicolumn{1}{l|}{$0.81\pm$0.19}    & \multicolumn{1}{l|}{$0.99\pm0.01$}     & \multicolumn{1}{l|}{$0.95\pm0.04$}        & \multicolumn{1}{l|}{$0.74\pm0.31$}         & \multicolumn{1}{l|}{$0.98\pm$0.02}     & $0.85\pm0.14$                \\ \hline
%Pickup Net                                                 &  $0.96\pm0.06$                           & \multicolumn{1}{l|}{$0.77\pm0.16$}    & \multicolumn{1}{l|}{$0.78\pm0.14$}     & \multicolumn{1}{l|}{$0.79\pm0.16$}        & \multicolumn{1}{l|}{$0.78\pm0.2$}         & \multicolumn{1}{l|}{$0.78\pm0.14$}     &  $0.75\pm0.13$               \\ \hline
%State Machine                                              &   $0.92\pm0.08$                          & \multicolumn{1}{l|}{0.97$\pm$0.05}    & \multicolumn{1}{l|}{$0.99\pm0.005$}     & \multicolumn{1}{l|}{$0.99\pm0.01$}        & \multicolumn{1}{l|}{$0.94\pm0.07$}         & \multicolumn{1}{l|}{$0.99\pm0.01$}     &  $0.96\pm0.03$               \\ \hline
%Vehicle Rental                                             &                             & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}     &                 \\ \hline
%Videoclub                                                  &                             & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}     &                 \\ \hline
%\textbf{All}                                                        &                             & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}     &                
%\end{tabular}
%\end{table*}

% To study the graph similarity we have used Graph Kernels... As explained before, for each domain we have generated 30 instances. Then, we have compared the similarity of the graph structure of very pair of instances. A value of 1 means that the two instances have a graph with the same structure and a 0 that the graph structure is different. The comparison of all the instances with each other results in a symmetric matrix with all the values in its diagonal 1. All these matrices are available in our anonymous repository~\cite{repo}. For each domain matrix (focusing only on the values above the main diagonal), we have calculated the average of its values and standard deviation. This gives us an idea of the average diversity of graph structures per domain... Table\ref{tab:graphSimilarity} shows this results. For the CoT strategy we have also reported on the diversity per category of instances.

% \todo{discuss somewhere in the paper the semantic coherence - right now we are discussing the semantics at the attribute value level but in the future we would have to do it at the model level (i.e., a Finish bank has customer with Finish names}

\subsubsection{RQ3 - Semantic diversity}
Table~\ref{tab:semantic-similarity} summarizes the calculated semantic diversity scores within and across instances. %Note, that the more semantically diverse two instances are, the closer their diversity metric is to 1; identical instances would yield a score of 0 (cf.\ Section~\ref{sec:eval-metrics}). 
Please note that the table shows the diversity metrics for both prompting strategies combined as there was no significant difference in the per-strategy results (which are provided in~\cite{repo}). The results clearly show that the two strategies are very effective in generating semantically diverse instances across all ten domains. Especially, the fact that the generated instances hardly had duplicate exact strings in the property values within instances and even across instances is intriguing. %Generally, there is no significant difference in the similarity within and across instances.

%\begin{table*}[]
%\caption{Semantic Similarity}
%\label{tab:semantic-diversity}
%\begin{tabularx}{\textwidth}{l|Y|Y|Y||Y|Y|Y}
%\multirow{3}{*}{Domain} & \multicolumn{3}{c||}{Diversity within instances} & \multicolumn{3}{c}{Diversity across instances} \\ 
%\cmidrule{2-7} 
% & \multirow{2}{*}{Numeric} & \multicolumn{2}{c||}{String} & \multirow{2}{*}{Numeric} & \multicolumn{2}{c}{String} \\ \cmidrule{3-4} \cmidrule{6-7} 
% & & Exact match & Norm. Lev. dist. & & Exact match & Norm. Lev. dist. \\ 
%\toprule
%Address Book     & -    & 0.0043 $\pm$ 0.0014& 0.1111 $\pm$ 0.007  & -    & 0.001 & 0.1019  \\ \midrule
%Bank    & 0.0031 $\pm$ 0.0172        & 0.0035 $\pm$ 0.0073& 0.0904 $\pm$ 0.0234 & 0.0148   & 0.0013& 0.0755  \\ \midrule
%Hotel Management & 0.0354 $\pm$ 0.0246        & 0.068 $\pm$ 0.0265 & 0.2423 $\pm$ 0.038  & 0.0249   & 0.0031& 0.1823  \\ \midrule
%Expenses& 0.1317 $\pm$ 0.3252        & 0.000 $\pm$ 0.000 & 0.1068 $\pm$ 0.0229 & 0.0326   & 0.004 & 0.1081  \\ \midrule
%Pickup Net       & 0.0528 $\pm$ 0.152& 0.000 $\pm$ 0.000 & 0.1209 $\pm$ 0.0184 & 0.0167   & 0.0036& 0.1234  \\ \midrule
%State Machine    & 0.0403 $\pm$ 0.0944        & 0.0013 $\pm$ 0.0036& 0.2377 $\pm$ 0.054  & 0.0594   & 0.0013& 0.1609  \\ \midrule
%Vehicle Rental   & 0.0132 $\pm$ 0.0207        & 0.000 $\pm$ 0.000 & 0.1244 $\pm$ 0.0289 & 0.0099   & 0.0011& 0.1177  \\ \midrule
%Videoclub        & 0.03 $\pm$ 0.0814 & 0.000 $\pm$ 0.000 & 0.1588 $\pm$ 0.0348 & 0.0459   & 0.0014& 0.1663  \\ \midrule
%\bottomrule
%\end{tabularx}
%\end{table*}

\begin{table*}[]
\vspace{-.3cm}
\caption{Cummulated semantic diversity results for the 600 generated model instances through the IL and CoT strategies}
\label{tab:semantic-similarity}
\begin{tabularx}{\textwidth}{l|Y|Y|Y||Y|Y|Y}
\multirow{3}{*}{Domain} & \multicolumn{3}{c||}{Diversity within instances} & \multicolumn{3}{c}{Diversity across instances} \\ 
\cline{2-7} 
 & \multirow{2}{*}{Numeric} & \multicolumn{2}{c||}{String} & \multirow{2}{*}{Numeric} & \multicolumn{2}{c}{String} \\ \cline{3-4} \cline{6-7} 
 & & Exact match & Norm. Lev. dist. & & Exact match & Norm. Lev. dist. \\ 
\hline
Address Book & - & 0.9957 $\pm$ 0.0014 & 0.8889 $\pm$ 0.0070 & - & 0.9990 & 0.8981 \\ 
\hline
Bank & 0.9969 $\pm$ 0.0172 & 0.9965 $\pm$ 0.0073 & 0.9096 $\pm$ 0.0234 & 0.9852 & 0.9987 & 0.9245 \\ 
\hline
Hotel Management & 0.9646 $\pm$ 0.0246 & 0.9320 $\pm$ 0.0265 & 0.7577 $\pm$ 0.0380 & 0.9751 & 0.9969 & 0.8177\\
\hline
Expenses& 0.8683 $\pm$ 0.3252 & 1.0000  $\pm$ 0.0000 & 0.8932 $\pm$ 0.0229 & 0.9674 & 0.9960 & 0.8919 \\ 
\hline
Pickup Net & 0.9472 $\pm$ 0.1520 & 1.0000 $\pm$ 0.0000 & 0.8791 $\pm$ 0.0184 & 0.9833 & 0.9964 & 0.8766 \\ 
\hline
State Machine & 0.9597 $\pm$ 0.0944 & 0.9987 $\pm$ 0.0036 & 0.7623 $\pm$ 0.0540 & 0.9406 & 0.9987 & 0.8391 \\ 
\hline
Vehicle Rental & 0.9868 $\pm$ 0.0207 & 1.0000 $\pm$ 0.0000 & 0.8756 $\pm$ 0.0289 & 0.9901 & 0.9989 & 0.8823\\ 
\hline
Videoclub & 0.9700 $\pm$ 0.0814 & 1.0000 $\pm$ 0.0000 & 0.8412 $\pm$ 0.0348 & 0.9541 & 0.9986 & 0.8337 \\
\hline
Football & 0.9741 $\pm$ 0.0224 & 0.9945 $\pm$ 0.0031 & 0.8541 $\pm$ 0.0101 & 0.9660 & 0.9990 & 0.8614 \\
\hline
Restaurant & 0.9803 $\pm$ 0.0165 & 0.9996 $\pm$ 0.0006 & 0.8733 $\pm$ 0.0093 & 0.9788 & 0.9995 & 0.8842 \\
\bottomrule
\end{tabularx}
Note that, according to formula \ref{formula:diversity}, the values are in the range [0..1]. The closer the values are to 1, the higher the diversity is.
\vspace{-.2cm}
\end{table*}

To better understand the generation of semantically diverse instances, Fig.~\ref{fig:instance-examples} visualizes one created instance of the Bank domain with the IL approach (left) and one generated by the CoT  approach (right) in the boundary scenario. 
It is worth noting that the IL approach generates different IBANs and BICs for the accounts. For the CoT boundary scenario, a smaller model is generated, which uses persons who just fulfill the age constraint, and one account has a relatively high balance compared to the ones generated by the IL approach. Fig.~\ref{fig:instance-examples_continued} shows further generated instances by CoT. The left model is generated for the edge scenario and the right model for the over-constraint scenario. For the former, persons with very high age values and special characters in their names are generated.% who also have special characters in their names. %\todo{actually, Guðmundur - not sure if we have here an ASCII encoding problem in the object diagrams....} 
For the latter, we get an instance that points out potential changes to the domain model. First, a balance may be also negative in case an overdraft facility is granted for an account. Furthermore, depending on the given country, persons under 18 years old may already have an account. %Interestingly, three person objects have the same last name. % if they have a regular income.   

\begin{figure*}[h!]
  \centering
  \begin{subfigure}{.59\textwidth}
      \includegraphics[width=.99\linewidth]{figs/BankInstanceInstructionLearning.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.33\textwidth}
      \centering
      \includegraphics[width=.99\linewidth]{figs/bankinstancegenCoTBoundary.pdf}
  \end{subfigure}
  \caption{Two generated Bank domain model instances, the left one following the Instruction Learning approach, the right one following the Chain-of-Thought approach in the boundary scenario.}
  \label{fig:instance-examples}
  \vspace{-.3cm}
\end{figure*}


\begin{figure*}[h!]
  \centering
  \begin{subfigure}{.35\textwidth}
      \includegraphics[width=.99\linewidth]{figs/fig4a.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.48\textwidth}
      \centering
      \includegraphics[width=.99\linewidth]{figs/fig4b.pdf}
  \end{subfigure}
  \caption{Two generated Bank domain model instances, the left one following the Chain-of-Thought approach in the edge scenario, the right one following the Chain-of-Thought approach in the over-constraint scenario.}
  \label{fig:instance-examples_continued}
  \vspace{-.3cm}
\end{figure*}

\begin{mdframed}[style=rqanswer,nobreak=true]
{\textbf{Answering RQ3:}} The two prompting strategies are very effective in creating semantically diverse model instances. The category-enhanced Chain-of-Thoughts approach was especially effective in exploring the boundaries of the instance space defined by the domain model multiplicities and constraints.
\end{mdframed}


\subsection{Threats to validity}
Next, we discuss the four threats to validity types from~\cite{WohlinRHCB12}. 

\subsubsection{Conclusion validity}
%Conclusion validity affects the ability to draw correct conclusion about the relations between the treatment and the outcome, i.e., how reasonable the conclusion is. Examples that influence this threat to validity include the choice of sample size, and the measurement of the experiment.

One threat to conclusion validity is that LLMs show non-deterministic behavior~\cite{song2024good}. To derive relevant results, we used several runs for producing instances and also checked for the robustness of the results. %, which is considered as best practice when using techniques that incorporate some randomness~\cite{ArcuriBriand2011}.

\subsubsection{Construct validity}
%Construct validity refers to the extent to which the experiment setting reflects the theory, i.e., whether the research/tests are well-constructed using established standards and methods. For example, whether the type of samples are representative of the population or not; or whether the number of classes taken reflects common experience.

Our evaluation consists of a relatively small dataset. However, we aimed to cover different cases of domain models that incorporate different modeling features. These cases mostly fit the requirements concerning educational purposes. Larger domain models and/or instance models may be required for other purposes, which is left as future work. Another construct validity threat is concerned with the realistic value checks. For this, we selected a subset of the available attributes in the domain models for which we can establish pragmatic ways to check if the values are actually realistic values. We used a combination of automated tests (for 11 values) and manual checks (for nine values) %We also acknowledge that some tests we performed may even check if the values are real values, but we only validated them for realistic values in our study. 
To reason about how close these values represent reality is only tested for some model elements. Finally, for diversity, we only reason about the differences of the values, however, we do not check if the values reflect different groups from a population etc. This aspect, of course, needs additional treatment in the future as LLMs may have been trained with biased data. 

\subsubsection{Internal validity}
% Internal validity checks whether the test or instrument measures what it is supposed to. This threat can affect the independent variable with respect to causality. That is, the results may indicate a causal relationship, although there is none.
Our work is also concerned with internal validity threats. First, the usage of GPT-4o may be influenced by our previous experiences, which have, of course, an impact on how the prompting strategies have been defined. Also, the interpretation of the domain models is performed from the author's viewpoint and experiences. Moreover, we only considered realistic values but did not check for precision and recall, which may allow us to deal with particular problems of LLMs, such as hallucinations. To deal with such issues, additional studies are required in the future. 

\subsubsection{External validity}
% This kind of threat limits the ability to generalize the results beyond the experiment context.
The fact that we have used a dataset covering diverse domains and models with different sizes and language features gives us some confidence that our results may be generalized to other cases. However, we cannot generalize our results for large domain models and/or instances as it is known that there is some performance penalty (and even some restrictions given the token limit of LLMs) when the size of these grows. Further research is needed here. In addition, we only used one particular LLM in one particular version, and thus, we cannot generalize for other LLMs. 
We also have to be careful with generalization with respect to specific terminology and openly available data for certain domains. Some may be more restricted or highly specialized niche domains, and thus, are not well-supported by existing LLMs.  





==> sections/old/approach-old.tex <==
\section{Approach}
\label{sec:approach}

In the following, we first introduce the preliminaries to our approach (\secref{sec:approach:prelim}) before detailing the two different strategies we implemented for LLM-based domain model instantiation (cf.\ Fig.~\ref{fig:learningstrategies}). 
The first strategy uses \textit{a single prompt with a combination of instruction learning and one-shot learning} (top of Fig.~\ref{fig:learningstrategies}; introduced in \secref{sec:approach:instruct-learn}), and the second strategy uses \textit{Chain-of-Thought (CoT) learning} (bottom of Fig.~\ref{fig:learningstrategies}; introduced in \secref{sec:approach:CoT-learn}). 
While the former uses only one prompt to request the LLM to generate model instances, the latter uses three prompts. The rationale behind exploring these two strategies is that the former is more efficient and sustainable as it uses fewer prompts while the latter has the potential to provide more diverse instances steered by asking for specific instance categories (see Section~\ref{sec:approach:CoT-learn}).

\subsection{Preliminaries}
\label{sec:approach:prelim}

For presenting class diagrams and object diagrams in a compact and comprehensible format to the LLMs, we have chosen the UML-based Specification Environment (USE) tool~\cite{GogollaBR07}. USE provides a textual syntax to represent domain models and comes with the SOIL language to define instances.
Listings~\ref{lst:domainModelUSE} and~\ref{lst:instanceModelUSE} show excerpts of the domain model and instance model of Fig.~\ref{fig:modeling-at-a-glance}, respectively. Note that the domain model in USE can be enriched with constraints written in OCL.

{\small
\begin{lstlisting}[language=USE,numbers=left,caption=Excerpt of the domain model represented as a class diagram in USE,captionpos=b,label=lst:domainModelUSE,basicstyle=\scriptsize,xleftmargin=1.2em]
model BankAccount
class Account
attributes
    iban: String
    balance : Real
end
class Person
attributes
    firstName:String
    lastName:String
    age : Integer
end [...]
association Ownership between
    Person [1..2] role owner
    Account [*] role accounts
end [...]
constraints
context Account inv AdultOwners:
    self.owner->forAll(p | p.age >= 18) [...]
\end{lstlisting}
}

{\small
\begin{lstlisting}[language=USE,numbers=left,caption=Excerpt of an instance model in SOIL,captionpos=b,label=lst:instanceModelUSE,basicstyle=\scriptsize,xleftmargin=1.2em]
!new Account('account1')
!account1.iban := 'ES6000491500051234567892'
!account1.balance := 9350.5
!new Person('person1')
!person1.age := 21
!person1.firstName := 'Lucia'
!person1.lastName := 'Martin'
!insert (person1, account1) into Ownership
\end{lstlisting}
}

\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{figs/Approach.png}
    \caption{Overview of the two instance generation strategies}
    \label{fig:learningstrategies}
\end{figure}

\subsection{Instance Generation by Instruction Learning}
\label{sec:approach:instruct-learn}

The top of Fig.~\ref{fig:learningstrategies} graphically depicts the steps to generate instances, a pseudo-code presentation is given by Algorithm~\ref{alg:algorithmSimple}. 
We use a single prompt that employs instruction learning. In this prompt, we provide detailed instructions about the task we ask the LLM to perform.
It has been discussed that, in general, LLMs do not perform well with low resource languages (languages which have limited data available for training) and domain-specific languages~\cite{joel_survey_2024}.
Specific text-based modeling languages such as SOIL fall into this category.
Hence, we combine instruction learning with one-shot learning. One-shot learning is a prompting technique in which the LLM is provided with a single example (shot) of what it is expected to produce. \andrei{One shot learning can provide the shot in the user prompt or in the system prompt. In our new prompts we provide it in the system prompt. We need to remove it from the algorithm and say that we added it in the system prompt} With this shot, our goal is to help the LLM learn about the particularities of the languages we are using, in our case USE and SOIL, helping the LLM to learn how the instances need to be generated, especially from a syntactic point of view. Therefore, we provide the LLM with an example (shot) of how the instantiation in a concrete scenario is done. % similarly to the examples in Listings~\ref{lst:domainModelUSE} and~\ref{lst:instanceModelUSE}. 


\begin{algorithm}[!h]
\scriptsize 
\DontPrintSemicolon
\textbf{Input:} domModel : Domain Model, shot : example of SOIL syntax, numInstances : number of instances to generate, maxChecks : maximum number of times a tentative instance will be checked before being added to the set of final instances \\
\textbf{Output:} set of instances \\
\textbf{def} run(domModel, shot, numInstances, maxChecks)
\Begin{
    \textit{instances} $\leftarrow$ \{\}\;
    openNewChat()\;
    \textit{tentativeInstance} $\leftarrow$ prompts(domModel, shot)\;
    \textit{instance} $\leftarrow$ checkConformance(tentativeInstance, domModel, maxChecks)\;
    add(instance, instances)\;
    \For {n $\in (2..numInstances]$} {
        \textit{tentativeInstance} $\leftarrow$ prompt(`nextInstance')\;
        \textit{instance} $\leftarrow$ checkConformance(tentativeInstance, domModel, maxChecks))\;
        add(instance, instances);
    }
    \nl\KwRet{$instances$}
}
\textbf{def} checkConformance(tentativeInstance, domModel, maxChecks)
\Begin{
    \textit{i} $\leftarrow$ 0\;
    \textit{sPass}, \textit{error} $\leftarrow$ syntaxCheckUSE(tentativeInstance, domModel)\;
    \While {not sPass and i < maxChecks} {
        \textit{tentativeInstance} $\leftarrow$ prompt(`correct', error)\;
        \textit{pass}, \textit{error} $\leftarrow$ syntaxCheckUSE(tentativeInstance, domModel)\;
        \textit{i}++\;
    }
    \If {sPass}{
        \textit{i} $\leftarrow$ 0\;
        \textit{cPass}, \textit{error} $\leftarrow$ conformanceCheckUSE(tentativeInstance, domModel)\;
        \While {not cPass and i < maxChecks} {
            \textit{tentativeInstance} $\leftarrow$ prompt(`correct', error)\;
            \textit{cPass}, \textit{error} $\leftarrow$ conformanceCheckUSE(tentativeInstance, domModel)\;
            \textit{i}++\;
        }   
    }
    \nl\KwRet{$tentativeInstance$}
}
\caption{Instance Generation using Instruction Learning and One-shot learning}
\label{alg:algorithmSimple}
\end{algorithm}

Our approach receives as input the domain model in textual USE format, \andrei{remove}the shot with an example of the instance model syntax in SOIL, and three input parameters: the number of instances to be created, and the maximum number of times the LLM is asked to correct an erroneously generated instance. 

Our approach starts by creating a single prompt following the template that Listing~\ref{lst:promptInstructionLearning} shows, where 
%\{\{size-desc\}\} in line 10 is to be parameterized by one of the following alternatives: NONE(""), SMALL(" with around 10 to 15 objects"), MEDIUM(" with around 16 to 50 objects"), and LARGE(" with around 51 to 100 objects"); 
\{\{classDiagram\}\} in line 11 is to be replaced by a class diagram in the textual USE format (cf.\ Listing~\ref{lst:domainModelUSE}); and \{\{syntaxExample\}\} in line 13 by a model instance in SOIL format (cf.\ Listing~\ref{lst:instanceModelUSE}) with a shot. 

\begin{lstlisting}[language=Prompt,breakindent=1.3em,numbers=left,caption=Prompt for instruction learning,captionpos=b,label=lst:promptInstructionLearning,basicstyle=\scriptsize,xleftmargin=1.2em]
System prompt:
Given a conceptual model expressed in the UML-based Specification Environment (USE), your task is to generate valid and realistic instances that conform to the provided model.
<requirements>
- Instances must be syntactically correct according to the USE syntax_reference.
- Avoid unnecessary comments and output the instance in plain text (i.e., not markdown).
- Make sure instances fulfill all the model constraints, and that multiplicities, relationships, and attributes are valid and realistic.
- Provide multiple instances with diverse data values and structure.
</requirements>
<syntax_reference>
{{syntaxExample}}
</syntax_reference>
User prompt:
Create an instance for the following domain model:
<domain_model>
{{classDiagram}}
</domain_model>
\end{lstlisting}

We have designed the syntax example shot such that it covers a good number of instance elements like comments, primitive data types, instantiation of objects and relations in USE. 
For space reasons, we cannot provide all the prompt templates for all the categories here, but they are all available in our online anonymous supplementary material repository~\cite{repo}. 

% \begin{lstlisting}[language=USE,numbers=left,caption=Syntax example,captionpos=b,label=lst:syntaxExample,basicstyle=\scriptsize,xleftmargin=1.2em]
% -- This is a comment example
% -- Primitive data types:
%     -- Integer i.e. 1, 2, 3, etc.
%     -- Real i.e. 1.0, 21.89, 322.05556, etc.
%     -- Boolean i.e. true or false
%     -- String i.e. 'Hello World'
% -- You can create instances with the following syntax:
% !new <instance type>('<instance name>')
% -- Example:
% !new Client('client1')
% !new Store('store4')
% -- You can assign values to attributes for a created instance with the following syntax:
% !<instance name>.<attribute name> := <value>
% -- Example for different data types:
% !client1.clientId := 1 -- For Integer
% !client1.balance := 1123.45 -- For Real
% !client1.name := 'John' -- For Strings
% !store4.available := true -- For Boolean
% -- You can create associations between instances with the following syntax:
% !insert (<instance name1>, <instance name2>) into <association name>
% -- Example:
% !insert (client1, store4) into ClientStore
% -- Custom data types usage:
%     -- dataType Location
%     -- operations
%     --   Location(x : Real, y : Real)
%     --   some other operations
%     -- end
% -- You can create custom data types by calling the constructor directly; in this case, the constructor of Location requires two arguments: x and y of type Real. So it can be used as follows:
% !store4.location := Location(14.0, 289.0)
% -- Enums usage:
%     -- enum Type { Clothes, Shoes }
% -- Can be used as follows:
% !store4.type := #Clothes
% \end{lstlisting}

To ensure diversity in the generated model instances, we exploit the ``memory'' of the LLM and ask for additional instances in the same chat. After the LLM generated one instance, we use the prompt described in Listing~\ref{lst:prompt-diverse} to ask the LLM to generate another instance instead of asking for all of them at once. We repeat this process as many times as the user has specified in the input parameter \texttt{numInstances} (see lines 9 to 13 in Algorithm~\ref{alg:algorithmSimple}). 

\begin{lstlisting}[language=Prompt,breakindent=1.3em,numbers=left,caption=Prompt for generating another instance,captionpos=b,label=lst:prompt-diverse,basicstyle=\scriptsize,xleftmargin=1.2em]
User prompt:
Please, generate another instance that is structurally and semantically different from the previous ones.
\end{lstlisting}

For each tentative instance generated by the LLM, we use USE to check the conformance to the class diagram (syntax and constraints) (lines 19 and 27 in Algorithm~\ref{alg:algorithmSimple}).
When a check fails, we use the following prompt (see Listing~\ref{lst:prompt-feedback}), where we provide the error that USE throws to help the LLM fix its mistake. We repeat this process until the instance passes the test or up to the maximum number of times that the user specified in the parameter \texttt{maxChecks} (lines 20 to 24 and 28 to 32 in Algorithm~\ref{alg:algorithmSimple}).

\begin{lstlisting}[language=Prompt,breakindent=1.3em,numbers=left,caption=Prompt for revising a tentative model instance,captionpos=b,label=lst:prompt-feedback,basicstyle=\scriptsize,xleftmargin=1.2em]
User prompt:
The last output is partially incorrect:
{{error}}
Please provide the complete corrected output.
\end{lstlisting}

\subsection{Instance Generation by Chain-of-Thought Learning}
\label{sec:approach:CoT-learn}
Chain-of-Thought (CoT)~\cite{Wei2022CoT} learning enables complex reasoning capabilities through intermediate reasoning steps. 
We use CoT combined with single-shot learning to further improve the results. 
We provide a visual representation of our algorithm at the bottom of Fig.~\ref{fig:learningstrategies} and its formalization in Algorithm~\ref{alg:algorithmCoT}.

\begin{algorithm}[h]
\scriptsize
\DontPrintSemicolon
\textbf{Input:} domModel : Domain Model, shot : example of SOIL syntax, categories : description of instance categories, numInstances : number of instances to generate of each category,  maxChecks : maximum number of times a tentative instance will be checked before being added to the set of final instances \\
\textbf{Output:} set of instances \\
\textbf{def} run(domModel, categories, shot, numInstances, maxChecks)
\Begin{
    \textit{instances} $\leftarrow$ \{\}\;
    openNewChat()\;
    \textit{modelDescription} $\leftarrow$ prompt(`analyze', domModel)\;
    \textit{scenarioDescriptions} $\leftarrow$ prompt(`genScenarios', categories, numInstances)\;
    \For {scenario in scenarioDescriptions} {
        openNewChat()\;
        \textit{tentativeInstance} $\leftarrow$ prompts(`genInstance', scenario, shot)\;
        \textit{instance} $\leftarrow$ checkConformance(tentativeInstance, domModel, maxChecks))\;
        add(instance, instances)\;
        \While {$ |instances| < numInstances$} {
            \textit{tentativeInstance} $\leftarrow$ prompt(`nextInstance')\;
            \textit{instance} $\leftarrow$ checkConformance(tentativeInstance, domModel, maxChecks))\;
            add(instance, instances)\;
        }
    }
    \nl\KwRet{$instances$}
}
\textbf{def} checkConformance(...)
\Begin{
    // Same as in Algorithm~\ref{alg:algorithmSimple}
}
\caption{Instance Generation using CoT}
\label{alg:algorithmCoT}
% \todo{make the description of the input parameters homogeneous between this algorith and the previous one}
\end{algorithm}

In addition to the inputs of the Instruction Learning strategy, the CoT strategy receives a list describing the categories of instances that the LLM is expected to generate. 
Our approach starts by providing the LLM with the domain model as input and asking it to generate a textual description in the natural language of the domain. This step aims to help improve the LLM's understanding of the domain to be modeled. 
The prompt we have designed is described in Listing~\ref{lst:prompt-analysis}.

\begin{lstlisting}[language=Prompt,breakindent=1.3em,numbers=left,caption=Prompt for analyzing a domain model,captionpos=b,label=lst:prompt-analysis,basicstyle=\scriptsize,xleftmargin=1.2em]
System prompt:
You are tasked with analyzing domain models represented as class diagrams and expressed in the UML-based specification environment using its native syntax.
You must adhere to the following requirements:
- Use very clear language.
- Do not overexplain, be concise.
- Multiplicities must be very clear and easy to understand.
You should follow the structure and requirements below:
## Description
Start by explaining the overall structure and purpose of the model.
### Components
Break down the components of the model (i.e., classes and attributes), describing each, their type and purpose.
## Relationships
Describe the relationships between the components of the model, dependencies and multiplicities (i.e., minimum and maximum number of instances of one class that can be associated with instances of another class). Describe the multiplicities at both association ends.
## Invariants
Define the invariants that apply to the model (i.e., those constraints that must be fulfilled).
User prompt:
Analyze the following UML class diagram:
{{classDiagram}}
\end{lstlisting}

Then, we ask the LLM to generate, in natural language and for the domain model provided, \texttt{numInstances} characteristic model instances that fall into a specific \textit{category}. The list of categories is related to test-driven development research that aims to develop comprehensive test cases for software systems.
\begin{itemize}
    \item \emph{Base scenario:} standard, typical, or common scenario in which each class and relationship is present in the instance at least once if applicable.%\todo{the question is if a base scenario can be a complex scenario - imagine a complex application domain which just consists of complex examples? Maybe we have to differentiate the two a bit more}
    \item \emph{Complex scenario:} complex scenario that contains multiple interrelated entities and/or entities that are involved in multiple constraints.
    \item \emph{Boundary scenario:} scenario that focuses on the extreme upper or lower limits of valid input ranges, such as limits of multiplicities, empty collections, etc.%\todo{this sounds related to the edge scenario - at least what I know from software testing...}
    \item \emph{Edge scenario:} scenario in which the system behaves within but at the limit of the expected behavior, i.e., scenarios that are unusual or unlikely in real-life but possible according to the syntax and semantics of the model. Note that while the boundary case focuses on the syntactic boundaries of multiplicities, the edge scenario explores semantically boundary cases such as a bank with zero accounts or a shopping cart with 2000 unique items.%\dominik{is this what we mean Lola and Manuel?}\lola{yes, we want to identify scenarios that are that are wellformed and valid but that are not common in real life. For instance, A bank with zero accounts but with a capital of 3 billion, A person that is 150 years old (as long as this doesnt violate any constraint), A shopping cart with hundreds of different items, each item with a price of over 2000 euros.}
     %\todo{I find this category very interesting and helpful for modelers. Impossible should result into additional constraints - seems to be underspecification then. Unlikely is maybe different but very interesting to know...}
    \item \emph{Over-constraint detection:} scenario that represents a real-life situation that is logically valid but violates the model's multiplicities or constraints, exposing overly restrictive or unrealistic restrictions. %\todo{again, this category is very interesting and somehow the opposite to the previous one...}
\end{itemize}

The prompt we use is:

\begin{lstlisting}[language=Prompt,breakindent=1.3em,numbers=left,caption=System prompt,captionpos=b,label=lst:prompt-system,basicstyle=\scriptsize,xleftmargin=1.2em]
System prompt:
Your task is to generate a complete and diverse instance, in plain English, for a given category and based on a provided domain model description. The instance must adhere to these requirements:
- Be self-contained: Include all required attributes, relationships, and related entities in full detail.
- Conform to the model: Fulfill the constraints, multiplicities, relationships, and attributes defined in the class diagram model.
- Understand the context: Ensure that its attributes and relationships are relevant.
- Avoid duplication of instances: Take into consideration those instances previously built to avoid redundancy.
- Semantic diversity: From a semantic point of view, incorporate varied scenarios, including regional, linguistic, or cultural differences.
- Structural diversity: Include instances with different numbers of elements, different numbers of relationships and complexity, and create varied examples by changing entity attributes.
User prompt:
# Domain model description:
{{modelDescription}}
# Category:
{{categoryPrompt}}
\end{lstlisting}

For space reasons, we cannot provide all the prompt templates for all the categories here -- they are all available in~\cite{repo}. For illustration purposes, the prompt we have used for the category \emph{boundary scenario} is as follows:

\begin{lstlisting}[language=Prompt,breakindent=1.3em,numbers=left,caption=Prompt for the category boundary scenario,captionpos=b,label=lst:prompt-boundaryInstances,basicstyle=\scriptsize,xleftmargin=1.2em]
# Category: Boundary Instances
Create a boundary case instance. This is an instance that focuses on the extreme upper or lower limits of valid input ranges. For example:
- Upper or lower limits of multiplicities.
- For numbers in a range, the minimum and maximum valid values.
- Empty collections when possible, i.e., when they do not violate the semantics of the model or its constraints.
\end{lstlisting}

For each of the scenario descriptions generated by the LLM, we use the following prompt to ask the LLM to create an instance using the SOIL syntax. For this, we provide the example that Listing~\ref{lst:instanceModelUSE} presents.

\begin{lstlisting}[language=Prompt,breakindent=1.3em,numbers=left,caption=Prompt for the generation of a model instance,captionpos=b,label=lst:prompt-instantiator,basicstyle=\scriptsize,xleftmargin=1.2em]
System prompt:
You are tasked with creating instances of a domain model in the UML-based Specification Environment (USE). You will receive:
1. The UML class diagram that the instance conforms to
2. A sample syntax of a model instantiation
3. A description of the instance that needs to be created
Your goal is to generate these instances based on the provided description, adhering strictly to these requirements:
- The output must be in plain text, with no additional comments, descriptions, or explanations.
- Ensure that the created instance adheres to the provided description.
- Follow the syntax sample provided, without deviation.
- Take into account previously created instances to avoid using duplicate naming.
User prompt:
# UML class diagram:
{{classDiagram}}
# Syntax example of instances creation:
{{syntaxExample}}
# Instance description:
Create the instance according to this specification:
{{scenario}}
\end{lstlisting}

Like for the simple-prompt strategy, we use USE to perform conformance checks and corrections (when needed) before adding the generated instance to the output set of instances.

\subsection{Tool Support}
We developed a Java-based tool leveraging LangChain4j\footnote{\url{https://docs.langchain4j.dev/}} and the UML-based Specification Environment Tool (USE)~\cite{GogollaBR07} to check syntactic and conformance errors. Throughout our preliminary experiments, we evaluated multiple LLMs, including GPT-4o, DeepSeek R3, and Gemini 2.0. \andrei{Which one will we we show? GPT4o, GPT52, both?} Ultimately, we selected gpt-4o-2024-08-06 with default hyperparameters\footnote{\url{https://platform.openai.com/docs/models/gpt-4o}} as our model of choice due to its widespread industry adoption, its reasonable speed, and its initial performance using a variant of the banking domain model\footnote{Results of this initial assessment of different LLMs is provided in~\cite{repo}}.
It should be noted that although we used the described tools, the proposed approach remains agnostic to the programming language, the selected libraries and LLM, which is crucial given the rapid evolution of LLMs.

==> tables/old/old-errors.tex <==
% % \begin{table*}[]
% % \caption{Realism results for model instances generated through our Instruction Learning (IL) and Chain of Thought (CoT) strategies}
% % \label{tab:results}
% %   \centering
% %   \scriptsize
% % \setlength{\tabcolsep}{2pt}
% % \renewcommand{\arraystretch}{1.05}
% % \begin{tabularx}{\textwidth}{@{}>{\raggedright\arraybackslash}p{1.65cm}|*{6}{>{\centering\arraybackslash}p{0.95cm}|}>{\raggedright\arraybackslash}X|>{\raggedright\arraybackslash}X@{}}
% % \multicolumn{1}{l|}{Domain} & \multicolumn{6}{c|}{Realism rate by LLM-as-a-judge\textsuperscript{2}} & \multicolumn{2}{c}{\textit{Realistic Checks} -- Real Checks}  \\ 
% % & IL & \multicolumn{5}{c|}{CoT category\textsuperscript{3}} & \multicolumn{1}{c|}{IL} & \multicolumn{1}{c}{CoT} \\
% % & & Base & Complex & \shortstack{Bound-\\ary} & Edge & \shortstack{Over-\\constraint} & & \\
% % \hline
% % Address Book & 20.0\% & 16.7\% & 100\% & 50.0\% & 16.7\% & 16.7\% & \textit{Phone: 0/201}; \textit{Website: 85/201}; \textit{Emails: 0/201}; Real address: 82/166 
% % & 
% % \textit{Phone: 5/178}; \textit{Website: 14/178}; \textit{Emails: 10/178}; Real address: 128/197 \\ 
% % \hline
% % Bank & 90.0\% & 100\% & 83.3\% & 16.7\% & 0\% & 16.7\% & Real IBAN: 106/141; \textit{IBAN: 0/141}; \textit{BIC: 1/63}; \textit{Country: 0/63} & Real IBAN: 106/143; \textit{IBAN: 6/143}; \textit{BIC: 1/79}; \textit{Country: 0/79} \\ 
% % \hline
% % \begin{tabular}[c]{@{}l@{}}Hotel\\ Management\end{tabular} & 90.0\% & 100\% & 83.3\% & 0\% & 0\% & 33.3\% & \textit{Check in \textless{} Start date: 0/27}; \textit{Check out \textgreater{} End date: 0/27} & \textit{Check in \textless{} Start date: 0/32}; \textit{Check out \textgreater{} End date: 1/32} \\
% % \hline
% % Expenses & 33.3\% & 66.7\% & 100\% & 50.0\% & 0\% & 33.3\% & \textit{Start date \textgreater{}\ End date: 0/50} & \textit{Start date \textgreater{}\ End date: 3/62} \\ 
% % \hline
% % Pickup Net & 83.3\% & 100\% & 100\% & 16.7\% & 0\% & 16.7\% & Real address: 19/172; \textit{Lat/Long for address: 0/153}; X username: 0/80 & Real address: 134/199; \textit{Lat/Long for address: 1/65}; X username: 11/79 \\
% % \hline
% % State Machine & 73.3\% & 66.7\% & 66.7\% & 50.0\% & 50.0\% & 16.7\% &  &  \\
% % \hline
% % \begin{tabular}[c]{@{}l@{}}Vehicle\\ Rental\end{tabular} & 36.7\% & 66.7\% & 16.7\% & 0\% & 0\% & 0\% & Real address: 30/187; License plate: 50/115; Home phone: 0/48 & Real address: 46/172; License plate: 15/119; Home phone: 0/47 \\
% % \hline
% % Videoclub & 96.7\% & 100\% & 83.3\% & 50.0\% & 0\% & 16.7\% & Production title: 101/124; \textit{Production types\textsuperscript{1}: 10/23}; \textit{Genre: 2/6}; \textit{Actors: 38/39}; \textit{Release year \textgreater{} Rental year: 4/23} & 
% % Production title: 162/168; \textit{Production types\textsuperscript{1}: 2/6}; \textit{Genre: 3/3}; \textit{Actors: 10/10}; \textit{Release year \textgreater{} Rental year: 0/4} \\  
% % \hline
% % Football & 96.7\% & 100\% & 100\% & 100\% & 0\% & 50.0\% & \textit{Dates: 0/1063} & \textit{Dates: 29/1284}\\
% % \hline
% % Restaurant & 96.7\% & 50.0\% & 16.7\% & 50.0\% & 0\% & 16.7\% & \textit{Dates: 0/395}; \textit{Phone number: 0/395} & \textit{Dates: 0/463}; \textit{Phone number: 0/462}\\
% % \bottomrule
% % \end{tabularx}
% % \begin{minipage}{\textwidth}
% % \raggedright
% % \textsuperscript{1} For valid productions only.
% % \textsuperscript{2} Percentage of instances judged realistic by the LLM-as-a-judge.
% % \textsuperscript{3} Each CoT category contains six instances per domain; ``over-constraint'' denotes the deliberately invalid category.
% % \end{minipage}
% % \vspace{-.3cm}
% % \end{table*}


% \begin{table*}[t]
% \caption{Realism results for model instances generated through our Instruction Learning (IL) and Chain of Thought (CoT) strategies}
% \label{tab:results}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.12}
% \begin{tabularx}{\textwidth}{@{}>{\raggedright\arraybackslash}p{2.45cm}*{6}{>{\raggedleft\arraybackslash}p{0.95cm}}*{2}{>{\raggedright\arraybackslash\everypar{\hangindent=0.7em\hangafter=1\relax}}X}@{}}
% \toprule
% \multirow{3}{*}{Domain}
%   & \multicolumn{6}{c}{Realism rate by LLM-as-a-judge\textsuperscript{2}}
%   & \multicolumn{2}{c}{Successful realism checks} \\
% \cmidrule(lr){2-7}\cmidrule(lr){8-9}
% & \multicolumn{1}{c}{\multirow{2}{*}{IL}}
%   & \multicolumn{5}{c}{CoT category}
%   & \multicolumn{1}{Y}{\multirow{2}{*}{IL}}
%   & \multicolumn{1}{Y}{\multirow{2}{*}{CoT\textsuperscript{4}}} \\
% \cmidrule(lr){3-7}
% & & \multicolumn{1}{c}{Base} & \multicolumn{1}{c}{Complex}
%   & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Bound-\\ary\end{tabular}}
%   & \multicolumn{1}{c}{Edge}
%   & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Over-\\constraint\end{tabular}}
%   & & \\
% \midrule
% Address Book & 20.0\% & 16.7\% & 100\% & 50.0\% & 16.7\% & 16.7\%
%   & Phone: 201/201\par  Website: 116/201\par  Emails: 201/201\par  Address(API): 84/166
%   & Phone: 173/178\par  Website: 164/178\par  Emails: 168/178\par  Address(API): 69/197 \\
% \midrule
% Bank & 90.0\% & 100\% & 83.3\% & 16.7\% & 0\% & 16.7\%
%   & IBAN(API): 35/141\par  IBAN: 141/141\par  BIC: 62/63\par  Country: 63/63
%   & IBAN(API): 37/143\par  IBAN: 137/143\par  BIC: 78/79\par  Country: 79/79 \\
% \midrule
% Hotel Management & 90.0\% & 100\% & 83.3\% & 0\% & 0\% & 33.3\%
%   & Check in \textless{} Start date: 27/27\par  Check out \textgreater{} End date: 27/27
%   & Check in \textless{} Start date: 32/32\par  Check out \textgreater{} End date: 31/32 \\
% \midrule
% Expenses & 33.3\% & 66.7\% & 100\% & 50.0\% & 0\% & 33.3\%
%   & Start date \textgreater{} End date: 50/50
%   & Start date \textgreater{} End date: 59/62 \\
% \midrule
% Pickup Net & 83.3\% & 100\% & 100\% & 16.7\% & 0\% & 16.7\%
%   & Address(API): 153/172\par  Lat/Long(API)\textsuperscript{3}: 153/153\par  X username: 80/80
%   & Address(API): 65/199\par  Lat/Long(API)\textsuperscript{3}: 64/65\par  X username: 68/79 \\
% \midrule
% State Machine & 73.3\% & 66.7\% & 66.7\% & 50.0\% & 50.0\% & 16.7\% & & \\
% \midrule
% Vehicle Rental & 36.7\% & 66.7\% & 16.7\% & 0\% & 0\% & 0\%
%   & Address(API): 157/187\par  License plate: 65/115\par  Home phone: 48/48
%   & Address(API): 126/172\par  License plate: 104/119\par  Home phone: 47/47 \\
% \midrule
% Videoclub & 96.7\% & 100\% & 83.3\% & 50.0\% & 0\% & 16.7\%
%   & Title(API): 23/124\par  Type(API)\textsuperscript{1}: 13/23\par  Genre(API): 4/6\par  Actors(API): 1/39\par  Release(API) \textgreater{} Rental: 19/23
%   & Title(API): 6/168\par  Type(API)\textsuperscript{1}: 4/6\par  Genre(API): 0/3\par  Actors(API): 0/10\par  Release(API) \textgreater{} Rental: 4/4 \\
% \midrule
% Football & 96.7\% & 100\% & 100\% & 100\% & 0\% & 50.0\%
%   & Dates: 1063/1063
%   & Dates: 1255/1284 \\
% \midrule
% Restaurant & 96.7\% & 50.0\% & 16.7\% & 50.0\% & 0\% & 16.7\%
%   & Dates: 395/395\par  Phone number: 395/395
%   & Dates: 463/463\par  Phone number: 462/462 \\
% \bottomrule
% \end{tabularx}

% \medskip
% \begin{minipage}{\textwidth}
% \raggedright
% \footnotesize
% \textsuperscript{1} Movie or series, for valid productions only.
% \textsuperscript{2} Percentage of instances judged realistic by the LLM-as-a-judge.
% \textsuperscript{3} Latitude and longitude for matched address.
% \textsuperscript{4} CoT counts include the over-constraint instances results. That category asks for a real-life situation that is valid in practice but over-constrained by multiplicities or constraints.
% \end{minipage}
% \vspace{-.2cm}
% \end{table*}





% ----- 

% \begin{table*}[]
% \caption{Realism results for model instances generated through our Instruction Learning (IL) and Chain of Thought (CoT) strategies}
% \label{tab:results}
%   \centering
%   \scriptsize
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.05}
% \begin{tabularx}{\textwidth}{@{}>{\raggedright\arraybackslash}p{1.65cm}|*{6}{>{\centering\arraybackslash}p{0.95cm}|}>{\raggedright\arraybackslash}X|>{\raggedright\arraybackslash}X@{}}
% \multicolumn{1}{l|}{Domain} & \multicolumn{6}{c|}{Realism rate by LLM-as-a-judge\textsuperscript{2}} & \multicolumn{2}{c}{\textit{Realistic Checks} -- Real Checks}  \\ 
% & IL & \multicolumn{5}{c|}{CoT category\textsuperscript{3}} & \multicolumn{1}{c|}{IL} & \multicolumn{1}{c}{CoT} \\
% & & Base & Complex & \shortstack{Bound-\\ary} & Edge & \shortstack{Over-\\constraint} & & \\
% \hline
% Address Book & 20.0\% & 16.7\% & 100\% & 50.0\% & 16.7\% & 16.7\% & \textit{Phone: 0/201}; \textit{Website: 85/201}; \textit{Emails: 0/201}; Real address: 82/166 
% & 
% \textit{Phone: 5/178}; \textit{Website: 14/178}; \textit{Emails: 10/178}; Real address: 128/197 \\ 
% \hline
% Bank & 90.0\% & 100\% & 83.3\% & 16.7\% & 0\% & 16.7\% & Real IBAN: 106/141; \textit{IBAN: 0/141}; \textit{BIC: 1/63}; \textit{Country: 0/63} & Real IBAN: 106/143; \textit{IBAN: 6/143}; \textit{BIC: 1/79}; \textit{Country: 0/79} \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}Hotel\\ Management\end{tabular} & 90.0\% & 100\% & 83.3\% & 0\% & 0\% & 33.3\% & \textit{Check in \textless{} Start date: 0/27}; \textit{Check out \textgreater{} End date: 0/27} & \textit{Check in \textless{} Start date: 0/32}; \textit{Check out \textgreater{} End date: 1/32} \\
% \hline
% Expenses & 33.3\% & 66.7\% & 100\% & 50.0\% & 0\% & 33.3\% & \textit{Start date \textgreater{}\ End date: 0/50} & \textit{Start date \textgreater{}\ End date: 3/62} \\ 
% \hline
% Pickup Net & 83.3\% & 100\% & 100\% & 16.7\% & 0\% & 16.7\% & Real address: 19/172; \textit{Lat/Long for address: 0/153}; X username: 0/80 & Real address: 134/199; \textit{Lat/Long for address: 1/65}; X username: 11/79 \\
% \hline
% State Machine & 73.3\% & 66.7\% & 66.7\% & 50.0\% & 50.0\% & 16.7\% &  &  \\
% \hline
% \begin{tabular}[c]{@{}l@{}}Vehicle\\ Rental\end{tabular} & 36.7\% & 66.7\% & 16.7\% & 0\% & 0\% & 0\% & Real address: 30/187; License plate: 50/115; Home phone: 0/48 & Real address: 46/172; License plate: 15/119; Home phone: 0/47 \\
% \hline
% Videoclub & 96.7\% & 100\% & 83.3\% & 50.0\% & 0\% & 16.7\% & Production title: 101/124; \textit{Production types\textsuperscript{1}: 10/23}; \textit{Genre: 2/6}; \textit{Actors: 38/39}; \textit{Release year \textgreater{} Rental year: 4/23} & 
% Production title: 162/168; \textit{Production types\textsuperscript{1}: 2/6}; \textit{Genre: 3/3}; \textit{Actors: 10/10}; \textit{Release year \textgreater{} Rental year: 0/4} \\  
% \hline
% Football & 96.7\% & 100\% & 100\% & 100\% & 0\% & 50.0\% & \textit{Dates: 0/1063} & \textit{Dates: 29/1284}\\
% \hline
% Restaurant & 96.7\% & 50.0\% & 16.7\% & 50.0\% & 0\% & 16.7\% & \textit{Dates: 0/395}; \textit{Phone number: 0/395} & \textit{Dates: 0/463}; \textit{Phone number: 0/462}\\
% \bottomrule
% \end{tabularx}
% \begin{minipage}{\textwidth}
% \raggedright
% \textsuperscript{1} For valid productions only.
% \textsuperscript{2} Percentage of instances judged realistic by the LLM-as-a-judge.
% \textsuperscript{3} Each CoT category contains six instances per domain; ``over-constraint'' denotes the deliberately invalid category.
% \end{minipage}
% \vspace{-.3cm}
% \end{table*}







==> tables/old/old-sizeGenInstances.tex <==
\begin{table}[h!]
\caption{Number of generated model elements}
\label{tab:sizeGenInstances}
\begin{tabularx}{\columnwidth}{l|YYY|YYY}
\multicolumn{1}{c|}{\multirow{2}{*}{Domain}}               & \multicolumn{3}{c|}{Instruction Learning}                                       & \multicolumn{3}{c}{Chain-of-Thought Learning}                                           \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{l|}{\#obj} & \multicolumn{1}{l|}{\#att} & \#assoc & \multicolumn{1}{l|}{\#obj} & \multicolumn{1}{l|}{\#att} & \#assoc \\ \hline
Address Book                                               & \multicolumn{1}{l|}{331}   & \multicolumn{1}{l|}{1023}  & 362     & \multicolumn{1}{l|}{415}   & \multicolumn{1}{l|}{1274}  & 470     \\ \hline
Bank                                                       & \multicolumn{1}{l|}{215}   & \multicolumn{1}{l|}{555}   & 386     & \multicolumn{1}{l|}{223}   & \multicolumn{1}{l|}{590}   & 347     \\ \hline
\begin{tabular}[c]{@{}l@{}}Hotel\\ Management\end{tabular} & \multicolumn{1}{l|}{232}   & \multicolumn{1}{l|}{757}   & 201     & \multicolumn{1}{l|}{325}   & \multicolumn{1}{l|}{971}   & 321     \\ \hline
Expenses                                                   & \multicolumn{1}{l|}{153}   & \multicolumn{1}{l|}{483}   & 150     & \multicolumn{1}{l|}{254}   & \multicolumn{1}{l|}{761}   & 282     \\ \hline
Pickup Net                                                 & \multicolumn{1}{l|}{272}   & \multicolumn{1}{l|}{453}   & 381     & \multicolumn{1}{l|}{438}   & \multicolumn{1}{l|}{739}   & 502     \\ \hline
State Machine                                              & \multicolumn{1}{l|}{323}   & \multicolumn{1}{l|}{323}   & 513     & \multicolumn{1}{l|}{476}   & \multicolumn{1}{l|}{476}   & 774     \\ \hline
Vehicle Rental                                             & \multicolumn{1}{l|}{125}   & \multicolumn{1}{l|}{712}   & 155     & \multicolumn{1}{l|}{200}   & \multicolumn{1}{l|}{1205}  & 293     \\ \hline
Videoclub                                                  & \multicolumn{1}{l|}{157}    & \multicolumn{1}{l|}{315}   & 156     & \multicolumn{1}{l|}{321}   & \multicolumn{1}{l|}{567}   & 274  \\  \hline
Football                                                  & \multicolumn{1}{l|}{866}    & \multicolumn{1}{l|}{2151}   & 897     & \multicolumn{1}{l|}{864}   & \multicolumn{1}{l|}{2021}   & 902  \\  \hline
Restaurant                                                  & \multicolumn{1}{l|}{370}    & \multicolumn{1}{l|}{1164}   & 340     & \multicolumn{1}{l|}{737}   & \multicolumn{1}{l|}{2173}   & 714  \\  
\end{tabularx}
\vspace{-.5cm}
\end{table}

==> tables/old/old-table-results.tex <==
\begin{table*}[]
\caption{Errors in model elements generated through our Instruction Learning (IL) and Chain of Thought (CoT) strategies}
\label{tab:results}
  \centering
  \scriptsize
\begin{tabularx}{\textwidth}{p{1.45cm}|c|P{.6cm}|c|c|X|X}
\multicolumn{1}{l|}{Domain} & \multicolumn{2}{c|}{Syntax errors} & \multicolumn{2}{c|}{Conformance errors} & \multicolumn{2}{c}{Semantic errors (Realistic Checks -- \textit{Real Checks})}  \\ 
& IL & CoT & IL & CoT & \multicolumn{1}{c|}{IL} & \multicolumn{1}{c}{CoT} \\
\hline
Address Book & 0 & 0 & 0 & 0 & Phone: 0/91; Website: 0/91; Emails: 0/91; Well-formed address: 0/89; \textit{Real address: 84/89} 
& 
Phone: 0/94; Website: 0/94; Emails: 0/94; Well-formed address: 0/105; \textit{Real address: 68/105} \\ 
\hline
Bank & 0 & 0 & 0 & 0 & \textit{Real IBAN: 83/90}; IBAN: 10/90; BIC: 1/31; \textit{Real Country: 0/31} & \textit{Real IBAN: 73/79}; IBAN: 0/79; BIC: 2/33; \textit{Real Country: 0/33} \\ 
\hline
Hotel Management & 0 & 0 & 0 & 6/261\textsuperscript{2} & \textit{Check in \textless{} Start date: 0/31}; \textit{Check out \textgreater{} End date: 0/31} & \textit{Check in \textless{} 
 Start date: 0/30}; \textit{Check out \textgreater{} End date: 1/31} \\
\hline
Expenses & 0 & 0 & 0 & 3/48\textsuperscript{3} & \textit{Start date \textgreater{}\ End date: 0/32} & \textit{Start date \textgreater{}\ End date: 0/30} \\ 
\hline
Pickup Net & 0 & 0 & 0 & 0 & Well-formed address: 0/62; \textit{Real address: 34/62}; \textit{Lat/Long for address: 62/62}; X username: 0/31 & Well-formed address: 0/114; \textit{Real address: 53/114}; \textit{Lat/Long for address: 54/114}; X username: 4/57 \\
\hline
State Machine & 0 & 0 & 0 & 0 & Semantic coherence: 0/30\textsuperscript{4} & Semantic coherence: 1/30\textsuperscript{4} \\
\hline
Vehicle Rental & 0 & 3/1698 & 0 & 0 & Well-formed address: 0/63; \textit{Real address: 51/63}; License plate: 0/31; Home phone: 0/16 & Well-formed address: 0/79; \textit{Real address: 59/79}; License plate: 0/64; Home phone: 0/23 \\
\hline
Videoclub & 0 & 0 & 0 & 0 & \textit{Production title: 30/63}; \textit{Production types\textsuperscript{1}: 14/33}; \textit{Genre: 9/19}; \textit{Actors: 33/33}; \textit{Release year \textgreater{} Rental year: 0/33} & 
\textit{Production title: 75/89}; \textit{Production types\textsuperscript{1}: 3/14}; \textit{Genre: 9/13}; \textit{Actors: 22/22}; Release year \textgreater{} Rental year: 1/12\\  
\hline
Football & 0 & 28/3784 & 0 & 
\begin{tabular}[c]{@{}l@{}}19/756\textsuperscript{2} \\10/96\textsuperscript{3}\end{tabular}
 & Dates: 0/360; Player names: 0/90; Club names: 0/60; Team names: 0/60; Competition names: 0/30 & 
Dates: 0/259; Player names: 0/69; Club names: 0/61; Team names: 0/66; Competition names: 0/30\\
\hline
Restaurant & 0 & 9/3618 & 0 & 
\begin{tabular}[c]{@{}l@{}}8/651\textsuperscript{2} \\ 6/96\textsuperscript{3}\end{tabular}
& Dates: 0/158; Phone number: 0/158; Person names: 0/190; Restaurant names: 0/30; Driver Licenses: 0/5; Menu items: 0/29; Food items: 0/1 & Dates: 0/244; Phone number: 0/200; Person names: 0/312; Restaurant names: 0/30; Driver Licenses: 28/28; Menu items: 0/49; Food items: 0/116\\
\bottomrule
\end{tabularx}
\flushleft\textsuperscript{1} For valid productions only \hspace{.3cm} \textsuperscript{2} Violation of multiplicities \hspace{.3cm} \textsuperscript{3} Violation of constraints \hspace{.3cm} \textsuperscript{4} For state machine models we checked the semantic coherence of the entire instance
\vspace{-.3cm}
\end{table*}


% \begin{table*}[]
% \caption{Results for the single prompt instruction learning strategy}
% \label{tab:resultsSimple}
% \begin{minipage}{\textwidth}
%   \centering
% \begin{tabular}{l|l|l|l|l}
% \multicolumn{1}{c|}{Domain}                                                     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Syntax\\ errors\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Conform.\\ errors\end{tabular}} & \multicolumn{1}{c}{Correct Domain Semantics}  \\ \hline\hline
% \multicolumn{1}{l|}{Address Book}                                                & 0 & 0      & \begin{tabular}[c]{@{}l@{}}Phone: 91/91 (100\%);Website: 91/91 (100\%); Emails: 91/91 (100\%);\\ Well-formed address: 89/89 (100\%); Real address: 5/89 (5.62\%)\end{tabular}                                                        \\ \hline
% \multicolumn{1}{l|}{Bank}                                                       & 0 & 0      & \begin{tabular}[c]{@{}l@{}}IBAN: 7 / 90 (7.78\%); BIC: 30/31 (96.77\%); Country: 31/31 (100\%)\end{tabular}                                                                                                                         \\ \hline
% \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Hotel\\ Management\end{tabular}} & 0 & 0 & checkIn>=startDate: 31/31 (100\%); checkOut<=endDate: 31/31 (100\%)                                                           \\\hline
% \multicolumn{1}{l|}{Expenses}                                                   & 0 & 0 & startDate < endDate: 32/32 (100\%)                                                           \\ \hline
% \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Pickup Net\end{tabular}}       & 0 & 0 & \begin{tabular}[c]{@{}l@{}}Well-formed address: 62/62 (100\%); Real address: 28 / 62 (45.16\%);\\Correct Lat/Long for address: 0/62 (0\%); Well-formed X (Twitter) username: 31/31 (100\%)\end{tabular}                                                            \\\hline
% \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}State\\ Machine\end{tabular}}    & 0 & 0 & -                                                           \\\hline
% \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Vehicle\\ Rental\end{tabular}}   & 0 & 0 & \begin{tabular}[c]{@{}l@{}}Well-formed address: 63/63 (100\%); Real address: 12/63 (19.05\%);\\License plate: 31/31 (100\%); Home phone: 16/16 (100\%) \end{tabular}                                                           \\\hline
% \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Videoclub\end{tabular}}      & 0 & 0 & \begin{tabular}[c]{@{}l@{}}Production title: 33/63 (52.38\%); For valid productions: Production types (movie /series):19/33 \\(57.58\%); Genre: 10/19 (52.63\%); Actors: 0/33 (0\%); Release year > Rental year: 33/33 (100.00\%); \end{tabular}    
% \end{tabular}
% \end{minipage}
% \end{table*}

% \begin{table*}[]
% \caption{Results for the CoT strategy}
% \label{tab:resultsCoT}
% \begin{minipage}{\textwidth}
%   \centering
% \begin{tabular}{l|l|l|l|l|l}
% \multicolumn{1}{c|}{Domain}                                & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Syntax\\ errors\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Conform. errors (excl.\\over-constraint detection)\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}Over-\\constraint\\ Detection\end{tabular} & \multicolumn{1}{c}{Correct Domain Semantics}                    \\ \hline\hline
% Address Book                                               & 0    & 0             &  No   & \begin{tabular}[c]{@{}l@{}}Phone: 94/94 (100\%);Website: 94/94 (100\%); Emails: 94/94 (100\%);\\ Well-formed address: 105/105 (100\%); Real address: 37/105 (35.24\%)\end{tabular}                                                                                     \\ \hline
% Bank                                                       & 0    & 0  & Yes \footnote{The constraint Account::positiveBalance fails as the LLM assumes there could be an account with a negative balance and it generated a test case where this happens} & IBAN: 5 / 79 (6.33\%); BIC: 29/33 (87.88\%); Country: 33/33 (100\%)                                                                                                                            \\ \hline
% \begin{tabular}[c]{@{}l@{}}Hotel\\ Management\end{tabular} & 0    & \begin{tabular}[c]{@{}l@{}}Mult: 6/261 (2.33\%);\\ Constraints: 0\end{tabular} &  Yes \footnote{Room reservation and Bill has multiplicity 1 in both ends, but the LLM assumes a reservation could be * in both ends which makes sense)}  & checkIn\textgreater{}=startDate: 30/30 (100\%); checkOut\textless{}=endDate: 29/31 (96.67\%)                                                \\ \hline
% Expenses                                                   & 0    & \begin{tabular}[c]{@{}l@{}}Mult: 0;\\ Constraints: 3/48 (6.25\%)\end{tabular}        &  Yes\footnote{constraint expenseSumOfBills fails}                                                                  & startDate \textless endDate: 30/30 (100\%)                         \\ \hline
% Pickup Net                                                 & 0    & 0  &Yes\footnote{Shipment::differentPickupAndDeliveryAddress fails because the model creates a scenario where the pickup and delivery address are the same... wrong}                                                                    & \begin{tabular}[c]{@{}l@{}}Well-formed address: 114/114 (100\%); Real address: 61 / 114 (53.51\%); Correct\\ Lat/Long for address: 60/114 (52.63\%); Well-formed X username: 53/57 (92.95\%)\end{tabular}    \\ \hline
% \begin{tabular}[c]{@{}l@{}}State\\ Machine\end{tabular}    & 0    & 0             &  Yes\footnote{it creates statemachines without start states (multiplicity violation)}                                                                  & -                                                                    \\ \hline
% \begin{tabular}[c]{@{}l@{}}Vehicle\\ Rental\end{tabular}   &

% \begin{tabular}[c]{@{}l@{}}3/1698\\(0.001\%)\end{tabular}
%     & 0             &  Yes\footnote{Multiplicity fail: RentalAgreement connected to 0 Vehicles. RentalAgreement connected to 0 offices. RentalAgreement connected to two customers (instead of 1)} &  \begin{tabular}[c]{@{}l@{}}Well-formed address: 79/79 (100\%); Real address: 20/79 (25.32\%);\\License plate: 64/64 (100\%); Home phone: 23/23 (100\%) \end{tabular}                                                                     \\ \hline
% Videoclub                                                  & 0    & 0             &  Yes\footnote{Production connected to 0 Actors} &  \begin{tabular}[c]{@{}l@{}}Production title: 14/89 (15.73\%); For valid productions: Production types\\ (movie /series):11/14 (78.57\%); Genre: 4/13 (30.77\%); Actors: 0/22 (0\%);\\Release year > Rental year: 11/12 (91.67\%); \end{tabular}                                                       
% \end{tabular}
% \end{minipage}
% \end{table*}
